Quantization-Aware Phase Retrieval

We address the problem of phase retrieval (PR) from quantized measurements. The goal is to reconstruct a signal from quadratic measurements encoded with a finite precision, which is indeed the case in many practical applications. We develop a rank-1 projection algorithm that recovers the signal subject to ensuring consistency with the measurement, that is, the recovered signal when encoded must yield the same set of measurements that one started with. The rank-1 projection stems from the idea of lifting, originally proposed in the context of PhaseLift. The consistency criterion is enforced using a one-sided quadratic cost. We also determine the probability with which different vectors lead to the same set of quantized measurements, which makes it impossible to resolve them. Naturally, this probability depends on how correlated such vectors are, and how coarsely/finely the measurements get quantized. The proposed algorithm is also capable of incorporating a sparsity constraint on the signal. An analysis of the cost function reveals that it is bounded, both above and below, by functions that are dependent on how well correlated the estimate is with the ground truth. We also derive the Cram\'er-Rao lower bound (CRB) on the achievable reconstruction accuracy. A comparison with the state-of-the- art algorithms shows that the proposed algorithm has a higher reconstruction accuracy and is about 2 to 3 dB away from the CRB. The edge, in terms of the reconstruction signal-to-noise ratio, over the competing algorithms is higher (about 5 to 6 dB) when the quantization is coarse.

==> QPR arxiv Oct1_2018/bibliography_thesis.tex <==
\begin{thebibliography}{999}
\newcommand{\enquote}[1]{``#1''}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\noopsort}[1]{}
\providecommand{\switchargs}[2]{#2#1}

%\bibitem{CIPIC}
%V. R. Algazi, R. O. Duda, D. M. Thompson and C. Avendano,
%\newblock  ``The CIPIC HRTF database,"
%\newblock in \emph{Proc. IEEE Workshop Appl. Sig. Proc. to Audio and Acoust.}, pp. 99--102, 2001.

%%%----------------------------------------
%Intro references
\bibitem{hvpoor_book}
H. V. Poor, \emph{An Introduction to Signal Detection and Estimation}., $2^{\text{nd}}$ Edition, Spronger-Verlang, 1994.


\bibitem{landweber}
L. Landweber, ``An iteration formula for Fredholm integral equations of the first kind," \emph{Amer. J. Math.}, vol. 73, pp. 615--624, 1951.

\bibitem{nonlin_landweber}
M. Hanke, A. Neubauer, and O. Scherzer, ``A convergence analysis of the Landweber iteration for nonlinear ill-posed problems," \emph{Numerische Mathematik}, Vol. 72, no. 1, pp. 21--37, 1995.

\bibitem{landweber_thesis}
T. Nikazad, ``The use of Landweber algorithm in image reconstruction," \emph{Link\"oping Studies in Sci. and Tech.}, Thesis no. 1311 (Link\"oping Universitet, Sweden), 2007. 

\bibitem{semi_conv_hansen}
T. Elfving, T. Nikazad, and P. C. Hansen, ``Semi-Convergence and Relaxation Parameters for a class of SIRT algorithms," \emph{Electronic Trans. Numerical Analysis}. vol. 37, pp. 321--336, 2010.


\bibitem{tikhonov_book1}
A. N. Tikhonov, A. V. Goncharsky, V. V. Stepanov, and A. G. Yagola, \emph{Numerical Methods for the Solution of Ill-Posed Problems.} Kluwer Academic Publishers, 1995.

\bibitem{tikhonov_book2}
A. N. Tikhonov, A. S. Leonov, A. G. Yagola, \emph{Nonlinear Ill-Posed Problems.} Chapman and Hall, 1998.


\bibitem{tv_reg_ref}
D. Strong and T.Chan, ``Edge-preserving and scale-dependent properties of total variation regularization," \emph{Inverse Problems}, vol. 19, pp. 165--187, 2003.

\bibitem{jain_iht}
P. Jain, A. Tewari, and P. Kar, ``On iterative hard thresholding methods for high-dimensional M-estimation," in \emph{Proc. Adv. in Neural Info. Process. Systems (NIPS)}, pp. 685--693, 2014. 

\bibitem{parikh_boyd_admm}
S. Boyd, N. Parikh, E. Chu, B. Peleato, and J. Eckstein, ``Distributed optimization and statistical learning via the alternating direction method of multipliers," 
\emph{Foundations and Trends in Mach. Learn.}, vol. 3, no. 1, pp. 1--122, 2011.

\bibitem{prox_grad_beck}
A. Beck and M. Teboulle, ``Gradient-based algorithms with applications to signal recovery problems," in \emph{Convex Optimization in Signal Process. and Comm.}, (D. Palomar and Y. Eldar, eds.), pp. 42--88, Cambridge University Press, 2010.

\bibitem{omp_guarantee}
J. Wang and B. Shim, ``On the recovery limit of sparse signals using orthogonal matching pursuit," \emph{IEEE Trans. Signal Process.},  vol. 60, no. 9, pp. 4973--4976, Sep. 2012. 


\bibitem{blumensath_iht}
T. Blumensath and M. E. Davies, ``Iterative hard thresholding for compressed sensing," \emph{Appl. Comput. Harmon. Anal.}, vol. 27, issue 3, pp. 265--274, 2009.

\bibitem{ds_annala_stat}
E. J. Cand\`es and T. Tao, ``The Dantzig Selector: Statistical estimation when $p$ is much larger than $n$," \emph{The Annals of Stat.}, vol. 35, no. 6, pp. 2313--2351, 2007.
%%%----------------------------------------
%Robust DL references
\bibitem{candes_cs_intro_2008}
E. J.~Cand\`es and M.~Wakin, ``An introduction to compressive sampling,'' {\em IEEE Signal Process. Mag.}, vol.~25, pp.~21 --30, Mar. 2008.

\bibitem{baraniuk_cs_tutorial}
R. Baraniuk, ``Compressive sensing," \emph{IEEE Signal Process. Mag.}, vol. 24, no. 4, pp. 118--121, Jul. 2007.

\bibitem{candes_tao_org}
E. J. Cand\`es, J. Romberg, and T. Tao, ``Robust uncertainty principles: Exact signal reconstruction from highly incomplete frequency information," \emph{IEEE Trans. Info. Theory,} vol. 52, no. 2, pp. 489--509, Feb. 2006.

\bibitem{donoho_it}
D. Donoho, ``Compressed sensing," \emph{IEEE Trans. Info. Theory}, vol. 52, no. 4, pp. 1289--1306, Apr. 2006.

\bibitem{elad_book}
M. Elad, \emph{Sparse and Redundant Representations: From Theory to Applications in Signal and Image Processing}. Springer, 2010.

\bibitem{rubinstein_dl_review}
R. Rubinstein, A. M. Bruckstein, and M. Elad, ``Dictionaries for sparse representation modeling," \emph{Proc. IEEE}, vol. 98, no. 6, pp. 1045--1057, Jun. 2010.

\bibitem{tosic_dl_review}
I. Tosic and P. Frossard, ``Dictionary learning," \emph{IEEE Signal Process. Mag.}, vol. 28, no. 2, pp. 27--38, Mar. 2011.

\bibitem{elad_ksvd_tip}
M. Elad and M. Aharon, ``Image denoising via sparse and redundant representations over learned dictionaries," \emph{IEEE Trans. Image Process.}, vol. 15, no. 12, pp. 3736--3745, Dec. 2006.

\bibitem{elad_ksvd_tsp}
M. Aharon, M. Elad, and A. Bruckstein, ``K-SVD: An algorithm for designing overcomplete dictionaries for sparse representation," \emph{IEEE Trans. Signal Process.}, vol. 54, no. 11, pp. 4311--4322, Nov. 2006.

\bibitem{arora_ksvd}
S. Arora, R. Ge, and A. Moitra, ``New algorithms for learning incoherent and over-complete dictionaries," \emph{J. Mach. Learn. Res.}, vol. 35, pp. 1--28, 2014. 

\bibitem{schnass_ksvd}
K. Schnass, ``On the identifiability of over-complete dictionaries via the minimization principle underlying K-SVD," \emph{Appl. and Comp. Harmonic Anal.}, vol. 37, issue 3, pp. 464--491, Nov. 2014. 

\bibitem{dai_simco}
W. Dai, T. Xu, and W. Wang, ``Simultaneous codeword optimization (SimCO) for dictionary update and learning," \emph{IEEE Trans. Signal Process.}, vol. 60, no. 12, pp. 6340--6353, Dec. 2012.

\bibitem{engan_mod}
K. Engan, S. O. Aase, and J. H. Husoy, ``Method of optimal directions for frame design," \emph{in   Proc. IEEE Intl. Conf. on Accoust., Speech, and Signal Process.}, pp. 2443--2446, Mar. 1999. 

\bibitem{yang_sr}
J. Yang, J. Wright, T. S. Huang, and Y. Ma, ``Image super-resolution via sparse representation," \emph{IEEE Trans. Image Process.}, vol. 19, no. 11, pp. 2861--2873, Nov. 2010.

\bibitem{sujit_inp}
S. Sahoo and W. Lu, ``Image in-painting using sparse approximation with adaptive window selection," in \emph{Proc. IEEE Intl. Symp. on Intell. Signal Process.}, pp. 1--4, Sep. 2011.

\bibitem{julien_imrest}
J. Mairal, M. Elad, and G. Sapiro, ``Sparse representation for color image restoration,"  \emph{IEEE Trans. Image Process.}, vol. 17, pp. 53--69, Jan. 2008.

\bibitem{zhang_cvpr}
Q. Zhang and B. Li, ``Discriminative K-SVD for dictionary learning in face recognition," in \emph{Proc. Conf. on Comp. Vis. and Pattern Recog.  (CVPR)}, pp. 2691--2698, 2010.

\bibitem{jiang_cvpr}
Z. Jiang, Z. Lin, and L. S. Davis, ``Learning a discriminative dictionary for sparse coding via label consistent K-SVD," in Proc. \emph{Proc. Conf. on Comp. Vis. and Pattern Recog.  (CVPR)}, pp. 1697--1704, 2011.

\bibitem{dtao_multiview_hessian}
W. Liu, D. Tao, J. Cheng, and Yuanyan Tang, ``Multiview Hessian discriminative sparse coding for image annotation," \emph{Elsevier Computer Vision and Image Understanding}, vol. 118, pp. 50--60, Jan. 2014.

\bibitem{dtao_group_sparse}
Y. Sun, Q. Liu, J. Tang, and D. Tao, ``Learning discriminative dictionary for group sparse representation," \emph{IEEE Trans. Image Process.}, vol. 23, no. 9, pp. 3816--3828, Sep. 2014.

\bibitem{liangyueli_elsevier}
L. Li, S. Li, and Y. Fu, ``Learning low-rank and discriminative dictionary for image classification," \emph{Elsevier Signal Process.}, vol. 32, no. 10, pp. 814--823, Oct. 2014.

\bibitem{yangfeixu_elsevier} 
Y. Xu, G. Bao, X. Xu, and Z. Ye, ``Single-channel speech separation using sequential discriminative dictionary learning," \emph{Elsevier Signal Process.}, vol. 106, pp. 134--140, Jan. 2015.

\bibitem{vahid_abolghasemi} 
V. Abolghasemi and S. Ferdowsi, ``EEGÐfMRI: Dictionary learning for removal of ballistocardiogram artifact from EEG," \emph{Elsevier Biomedical Signal Process. and Control}, vol. 18, pp. 186--194, Apr. 2015.


\bibitem{zgao_elsevier}
Z. Gao, H. Zhang, G. P. Xu, Y. B. Xue, and A. G. Hauptmann, ``Multi-view discriminative and structured dictionary learning with group sparsity for human action recognition," \emph{Elsevier Signal Process.}, vol. 112, pp. 83--97, Jul. 2015.

\bibitem{bishop_prml_book}
C.~M.~Bishop, \emph{Pattern Recognition and Machine Learning}. Springer, 2006.

\bibitem{dtao_geometric_mean}
D. Tao, X. Li, X. Wu, and S. J. Maybank, ``Geometric mean for subspace selection," \emph{IEEE Trans. Pattern Anal. Mach. Intell.}, vol. 31, no. 2, pp. 260--274, Feb. 2009.

\bibitem{kasiviswanathan_nips} 
S. P. Kasiviswanathan, H. Wang, A. Banerjee, and P. Melville, ``Online $\ell_1$ dictionary learning with application to novel document detection," in \emph{Proc. Adv. in Neural Info. Proc. Systems (NIPS)}, vol. 25, pp. 2267--2275, 2012.

\bibitem{spk_icassp}
S. P. Kasiviswanathan, ``Fast online $\ell_1$ dictionary learning algorithm for novel document detection," in \emph{Proc. IEEE Intl. Conf. on Accoust., Speech, and Signal Process.}, pp. 8585--8589, 2013.

\bibitem{tao_manhattan}
T. Liu and D. Tao, ``On the performance of Manhattan nonnegative matrix factorization," \emph{IEEE Trans. on Neural Networks and Learning Systems}, issue 99, Aug. 2015. 

\bibitem{lu_rdl}
C. Lu, J. Shi, and J. Jia, ``Online robust dictionary learning," in Proc. \emph{IEEE Conf. on Comp. Vis. and Patt. Recog.}, pp. 415--422, 2013.

\bibitem{online_DL}
J. Mairal, F. Bach, J. Ponce, and G. Sapiro, ``Online dictionary learning for sparse coding," in \emph{Proc. $26^{\text{th}}$ Annual Intl. Conf. on Machine Learning}, pp. 689--696, 2009.

\bibitem{wang_elsev}
S. Wang, Q. Liu, Y. Xia, P. Dong, J. Luo, Q. Huang, and D. D. Feng, ``Dictionary learning based impulse noise removal via $\ell_1-\ell_1$ minimization," \emph{Elsevier Signal Process.}, vol. 93, no. 9, pp. 2696--2708, Sep. 2013.  


\bibitem{tao_cauchy}
T. Liu and D. Tao, ``On the robustness and generalization of Cauchy regression," in Proc. \emph{IEEE Intl. Conf. on Information Science and Technology} (ICIST), pp. 100--105, Apr. 2014.  

\bibitem{daubechies_irls} 
I. Daubechies, R. DeVore, M. Fornasier, and C. S. G\"{u}nt\"{u}rk, ``Iteratively re-weighted least-squares minimization for sparse recovery," \emph{Comm. Pure and Appl. Math.}, vol. LXIII, pp. 1--38, 2010.


\bibitem {miosso_irls} 
C. J. Miosso, R. V. Borries, M. Arg\'{a}ez, L. Velazquez, C. Quintero, and C. M. Potes, ``Compressive sensing reconstruction with prior information by iteratively reweighted least-squares," \emph{IEEE Trans. Signal Process.}, vol. 57, no. 6, pp. 2424--2431, Jun. 2009.

\bibitem{endra_irls}
O. Endra and Gunawan, ``Comparison of $\ell_1$-minimization and iteratively reweighted least-squares-$\ell_p$-minimization for image reconstruction from compressive sensing," in \emph{Proc. Second Intl. Conf. on Advances in Computing, Control and Telecom. Tech.}, pp. 85--88, Dec. 2010.

\bibitem{tao_label_noise}
T. Liu and D. Tao, ``Classification with noisy labels by importance reweighting," \emph{IEEE Trans. Pattern Anal. and Mach. Intell.}, vol. 38, no. 3, pp. 447--461, Jul. 2015. 

\bibitem{grant_cvx} 
M. Grant and S. Boyd, ``CVX: Matlab software for disciplined convex programming," version 2.0 beta, Sep. 2013.


\bibitem{manopt}
N. Boumal, B. Mishra, P. A. Absil, and R. Sepulchre, ``ManOpt, a MATLAB toolbox for optimization on manifolds," \emph{J. Mach. Learning Res.}, vol. 15, pp. 1455--1459, 2014. 

\bibitem{brian_jeffs}
B. D. Jeffs and M. Gunsay, ``Restoration of blurred star field images by maximally sparse optimization," \emph{IEEE Trans. Image Process.}, vol. 2, no. 2, pp. 202--211, Apr. 1993.

\bibitem{ssim_paper_ref}
Z. Wang, A. C. Bovik, H. R. Sheikh, and E. P. Simoncelli, ``Image quality assessment: From error visibility to structural similarity," \emph{IEEE Trans. Image Process.}, vol. 13, no. 4, pp. 600--612, Apr. 2004.

\bibitem{bartlett_jmlr}
P. L. Bartlett and S. Mendelson, ``Rademacher and Gaussian complexities: Risk bounds and structural results," \emph{J. Mach. Learning Res.}, vol. 3, pp. 463--482, 2002.  

\bibitem{sudakov_ineq1}
V. N. Sudakov, ``Gaussian random processes and measures of solid angles in Hilbert space," \emph{Dokl. Akad. Nauk. SSR} vol. 197, pp. 412--415, 1971.

\bibitem{sudakov_ineq_proof}
S. Chatterjee, ``An error bound in the Sudakov-Fernique inequality," \emph{arXiv:math/0510424v1} Oct. 2005.

\bibitem{vahid}
V. Abolghasemi, S. Ferdowsi, and S. Sanei, ``Blind separation of image sources via adaptive dictionary learning," \emph{IEEE Trans. Image Process.}, vol. 21, no. 6, pp. 2921--2930, Jun. 2012.

\bibitem{SPK_nips}
S. P. Kasiviswanathan, H. Wang, A. Banerjee, and P. Melville, ``Online $\ell_1$-dictionary learning with application to novel document detection," in  \emph{Proc. Adv. in Neural Info. Proc. Systems (NIPS)}, vol. 3, pp. 2258--2266, 2012. 


\bibitem{bao}
C. Bao, J. Cai, and H. Ji, ``Fast sparsity-based orthogonal dictionary learning for image restoration," in \emph{Proc. IEEE Intl. Conf. on Comp. Vis.}, pp. 3384--3391, 2013.


%--------------------------------------
%DCDL references
\bibitem{rubinstein_double_sparsity}
R. Rubinstein, M. Zibulevsky, and M. Elad, ``Double sparsity: Learning sparse dictionaries for sparse signal approximation," \emph{IEEE Trans. Signal Process.}, vol. 58, no. 3, pp. 1553--1564, Mar. 2010.

\bibitem{naai}
N. Ai, J. Peng, X. Zhu, and X. Feng, ``SISR via trained double sparsity dictionaries," \emph{Multimedia Tools and Applications}, vol. 74, issue 6, pp. 1997--2007, Mar. 2015. 


\bibitem{online_DL_JMLR}
J. Mairal, F. Bach, J. Ponce, and G. Sapiro, ``Online learning for matrix factorization and sparse coding," \emph{J. Mach. Learn. Res.}, vol. 11, pp. 19--60, 2010.

\bibitem{cherian}
A. Cherian, S. Sra, and N. Papanikolopoulos, ``Denoising sparse noise via online dictionary learning," \emph{in Proc. IEEE Intl. Conf. on Accoust., Speech, and Signal Process.}, pp. 2060--2063, May 2011.

\bibitem{mackey}
L. Mackey, A. Talwalkar, and M. I. Jordan, ``Distributed matrix completion and robust factorization," \emph{J. Mach. Learn. Res.}, vol. 16, pp. 913--960, 2015.

\bibitem{chainais}
P. Chainais and C. Richard, ``Distributed dictionary learning over a sensor network," \emph{arXiv:1304.3568v1}, Apr. 2013.

\bibitem{liang_dist}
J. Liang, M. Zhang, X. Zeng, and G. Yu, ``Distributed dictionary learning for sparse representation is sensor networks," \emph{IEEE Trans. Image Process.}, vol. 23, no. 6, pp. 2528--2541, Jun. 2014.

\bibitem{dai_cluster}
T. Xu, W. Dai, and W. Wang, ``Fast dictionary learning algorithm via codeword clustering and hierarchical sparse coding," in \emph{Proc. $9^{\text{th}}$ IMA Intl. Conf. on Math. in Signal Process.}, Dec. 2012.

\bibitem{cormen_algo}
T. H. Cormen, C. E. Leiserson, R. L. Rivest, and C. Stein, \emph{Introduction to Algorithms $3^{\text{rd}}$ Edition}, The MIT Press, 2005.

\bibitem{tropp_omp}
J. A. Tropp and A. C. Gilbert, ``Signal recovery from random measurements via orthogonal matching pursuit," \emph{IEEE Trans. Info. Theory}, vol. 53, no. 12, pp. 4655--4666, Dec. 2007.


%------------------------------------------------------------
%SVR references
\bibitem{tropp_cosamp}
D.Needell and J.A.Tropp, ``CoSaMP: Iterative signal recovery from incomplete and inaccurate samples," \emph{Appl. and Comp. Harmonic Anal.}, vol. 26, issue 3, pp. 301--321, May 2009. 

\bibitem{donoho_bp_siam}
S. S. Chen, D. L. Donoho, and M. A. Saunders, ``Atomic decomposition by basis pursuit", \emph{SIAM J. of Sci. Comp.}, vol. 20, no. 1, pp. 33--61, Feb. 1997.


\bibitem{anal_ksvd1}
R. Rubinstein, T. Peleg, and M. Elad, ``Analysis K-SVD: A dictionary learning algorithm for the analysis sparse model," \emph{IEEE Trans. Signal Process.}, vol. 61, no. 3, pp. 661--677, Feb. 2013.

\bibitem{dai_analysis}
J. Dong, W. Wang, and W. Dai, ``Analysis SimCO: A new algorithm for analysis dictionary learning," in \emph{Proc. IEEE Intl. Conf. on Accoust., Speech, and Signal Process.}, pp. 7193--7197, May 2014.

\bibitem{ravishankar_TL1}
S. Ravishankar and Y. Bresler, ``Learning sparsifying transforms," \emph{IEEE Trans. Signal Process.}, vol. 61, no. 5, pp. 1072--1086, Mar. 2013.

\bibitem{ravishankar_TL2}
S. Ravishankar and Y. Bresler, ``$\ell_0$ sparsifying transform learning with efficient optimal updates and convergence guarantees," \emph{IEEE Trans. Signal Process.}, vol. 63, no. 9, pp. 2389--2404, May 2015.

\bibitem{ravishankar_online}
S. Ravishankar, B. Wen, and Y. Bresler, ``Online sparsifying transform learning--Part I: Algorithms," \emph{IEEE J. Selected Topics in Signal Process.}, vol. 9, no. 4, pp. 625--636, Jun. 2015.

\bibitem{transform_ksvd_ender}
E. M. Eksioglue and O. Bayir, ``K-SVD meets transform learning: Transform K-SVD," \emph{IEEE Signal Process. Lett.}, vol. 21, no. 3, pp. 347--351, Mar. 2014.

\bibitem{tight_frame_cai}
J.-F.  Cai, H. Ji, Z. Shen, and G.-B. Ye, ``Data-driven tight frame construction and image denoising," \emph{Appl. and Computational Harmonic Anal.}, vol. 37, issue 1, pp. 89-105, Jul. 2014. 

\bibitem{IPR_plumbley}
D. Barchiesi and M. D. Plumbley, ``Learning incoherent dictionaries for sparse approximation using iterative projections and rotations," \emph{IEEE Trans. Signal Process.}, vol. 61, no. 8, pp. 2055--2065, Apr. 2013.

\bibitem{opp_66}
P. H. Sch\"onemann, ``A generalized solution of the orthogonal Procrustes problem," \emph{Psychometrika}, vol. 31, issue 1, pp. 1--10, Mar. 1966.

\bibitem{ortho_sc}
H. Sch\"utze, E. Barth, and T. Martinetz, ``Learning efficient data representations with orthogonal sparse coding," \emph{IEEE Trans. Computational Imaging}, vol. 2, no. 3, pp.177--189, Sep. 2016.

\bibitem{bm3d_tip}
K. Dabov, A. Foi, V. Katkovnik, and K. Egiazarian, ``Image denoising by sparse 3D transform-domain collaborative filtering," \emph{IEEE Trans. Image Process.}, vol. 16, no. 8, pp. 2080--2095, 2007.


%------------------------------------------------------------
%LETnet/fLETnet references
\bibitem{candes_romberg_tao}
E. J. Cand\`es, J. Romberg, and T. Tao, ``Stable signal recovery from incomplete and inaccurate measurements," \emph{Comm. Pure and Appl. Math.} vol. 59 no. 8, pp. 1207--1223, 2006.

\bibitem{krizhevsky2012imagenet}
A. Krizhevsky, I. Sutskever, and G. E. Hinton, ``ImageNet classification
with deep convolutional neural networks," in \emph{Proc. Adv. in Neural Info. Process. Systems (NIPS)}, pp. 1097--1105, 2012.

\bibitem{resnet_ref}
K. He, X. Zhang, S. Ren, and J. Sun, ``Deep residual learning for image recognition," \emph{arXiv:1512.03385v1}, Dec. 2015.

\bibitem{beck_fista}
A. Beck and M. Teboulle, ``A fast iterative shrinkage-thresholding algorithm for linear inverse problems," \emph{SIAM J. Imaging Sci.}, vol. 2, no. 1, pp. 183--202, 2009.

\bibitem{sermanet2013overfeat}
P. Sermanet, D. Eigen, X. Zhang, M. Mathieu, R. Fergus, and Y. LeCun, ``Overfeat: Integrated recognition, localization and detection using
convolutional networks." in \emph{Proc. Intl. Conf. on Learning Representations}, 2014.

\bibitem{chen_murphy_deep_cnn}
 L. Chen, G. Papandreou, I. Kokkinos, K. Murphy, and A. L. Yuille, ``Semantic image segmentation with deep convolutional nets and fully
connected CRFs," \emph{arXiv:1412.7062}, 2014. 

\bibitem{hinton2010practical} 
G. Hinton, \emph{Neural Networks: Tricks of the Trade.} $2^{\text{nd}}$ Edition, Springer, Berlin 2012.

\bibitem{rifai2012disentangling}
S. Rifai, Y. Bengio, A. Courville, P. Vincent, and M. Mirza, ``Disentangling factors of variation for facial expression recognition," in \emph{ Proc. European Conf. on Comp. Vis.}, pp. 808--822, 2012.

\bibitem{sutskever2013training}
I. Sutskever, ``Training recurrent neural networks," \emph{Ph.D. dissertation, University of Toronto}, 2013.

\bibitem{ling2015deep}
Z. H. Ling, S. Y. Kang, H. Zen, A. Senior, M. Schuster, X. J. Qian, H. M. Meng, and L. Deng, ``Deep learning for acoustic modeling in parametric
speech generation: A systematic review of existing techniques
and future trends," \emph{IEEE Signal Process. Mag.}, vol. 32, no. 3, pp. 35--52, 2015.

\bibitem{graves2013speech}
A. Graves, A. Mohamed, and G. Hinton, ``Speech recognition with
deep recurrent neural networks," in \emph{Proc. IEEE Intl. Conf. on Acoustics, Speech and Signal Process.}, pp. 6645--6649, 2013.

\bibitem{rifai2012generative}
S. Rifai, Y. Bengio, Y. Dauphin, and P. Vincent, ``A generative process for sampling contractive auto-encoders," \emph{arXiv:1206.6434},
2012.

\bibitem{vincent2010stacked}
P. Vincent, H. Larochelle, I. Lajoie, Y. Bengio, and P. A. Manzagol, ``Stacked denoising auto-encoders: Learning useful representations in a
deep network with a local denoising criterion," \emph{J. Mach. Learn. Res.}, vol. 11, pp. 3371--3408, Dec. 2010.


\bibitem{goodfellow2012large} 
I. Goodfellow, A. Courville, and Y. Bengio, ``Large-scale feature learning with spike-and-slab sparse coding," in \emph{Proc. Intl. Conf. on Machine Learning}, 2012.

\bibitem{lecun_learned_ista}
K. Gregor and Y. LeCun, ``Learning fast approximations of sparse coding," in \emph{Proc. Intl. Conf. on Machine Learning}, 2010.

\bibitem{daubechies_ista}
I. Daubechies, M. Defrise, and C. De Mol, ``An iterative thresholding algorithm for linear inverse problems with a sparsity constraint," \emph{Comm. Pure Appl. Math.}, vol. 57, pp. 1413--1457, 2004.

\bibitem{deep_unfolding_2014}
J.~R.~Hershey, J.~L.~Roux, and F.~Weninger, ``Deep unfolding: Model-based inspiration of novel deep architectures," \emph{arXiv:1409.2575v4}, Nov. 2014.

\bibitem{schniter_lamp}
M. Borgerding, P. Schniter, and S. Rangan, ``AMP-Inspired Deep Networks for Sparse Linear Inverse Problems," \emph{IEEE Trans. Signal Process.}, vol. 65, no. 16, pp. 4293--4308, Aug. 2017.

\bibitem{kamilov_mmse_ista}
U.~S. Kamilov and H.~Mansour, ``Learning optimal nonlinearities for iterative thresholding algorithms,'' \emph{IEEE Signal Process. Letters}, vol.~23, no.~5, pp. 747--751, May 2016.

\bibitem{domke1_cvpr}
J. Domke, ``Parameter learning with truncated message-passing," in \emph{Proc. Comp. Vis. and Pattern Recog.}, pp. 2937--2943, 2011.

\bibitem{domke2_pami}
J. Domke, ``Learning graphical model parameters with approximate marginal inference," \emph{IEEE Trans. Pattern Anal. Mach. Intell.}, vol. 35, no. 10, pp. 24--54, 2013.

\bibitem{sprechmann_sapiro}
P. Sprechmann, A. M. Bronstein, and G. Sapiro, ``Learning efficient sparse and low rank models," \emph{IEEE Trans. Pattern Anal. Mach. Intell.}, vol. 37, no. 5, pp. 1821--1833, Sep. 2015.

\bibitem{wang_l0_encoder}
Z. Wang, Q. Ling, and T. S. Huang, ``Learning deep $\ell_0$ encoders," \emph{arXiv:1509.00153v2}, Nov. 2015.

\bibitem{xin_max_sparsity}
B. Xin, Y. Wang, W. Gao, and D. Wipf, ``Maximal sparsity with deep networks?," \emph{arXiv:1605.01636v2}, May 2016.

\bibitem{jin_et_al}
K. H. Jin, M. T. McCann, E. Froustey, and M. Unser, ``Deep convolutional neural network for inverse problems in imaging," \emph{IEEE Trans. Image Process.}, vol. 26, no. 9, pp. 4509--4522, Sep. 2017.   

\bibitem{ye_et_al}
J. C. Ye and Y. S. Han, ``Deep convolutional framelets: A general deep learning for inverse problems," \emph{arXiv:1707.00372v3}, Aug. 2017.

\bibitem{oktem1}
J. Adler and O. \"Oktem, ``Solving ill-posed inverse problems using iterative deep neural networks," \emph{arXiv:1704.04058v2}, May 2017.

\bibitem{oktem2}
J. Adler and O. \"Oktem, ``Learned primal-dual reconstruction," \emph{arXiv:1707.06474v1}, Jul. 2017.

\bibitem{blu_surelet}
T. Blu and F. Luisier, ``The SURE-LET approach to image denoising," \emph{IEEE Trans. Image Process.}, vol. 16, no. 11, pp. 2778--2786, 2007.


\bibitem{pan2013iterative}
H.~Pan and T.~Blu, ``An iterative linear expansion of thresholds for $\ell_1$-based image restoration,'' \emph{IEEE Trans. Image Process.}, vol.~22, no.~9, pp. 3715--3728, 2013.

\bibitem{martens_hfo}
J.~Martens, ``Deep learning via Hessian-free optimization,'' in \emph{Proc. $27^{\text{th}}$ Intl. Conf. Machine Learning}, pp. 735--742, 2010.

\bibitem{bengio_book}
I. Goodfellow, Y. Bengio, and A. Courville, \emph{Deep learning.}, available at \url{https://www.deeplearningbook.org}.

\bibitem{tibshirani_lasso}
R.Tibshirani, ``Regression shrinkage and selection via the LASSO," \emph{J. Royal Stat. Society, Series B}, vol. 58, no. 1, pp. 267--288, 1996.

\bibitem{parikh_boyd}
N. Parikh and S. Boyd, ``Proximal algorithms," \emph{Foundations and Trends in Opt.}, vol. 1, no. 3, pp. 123--231, 2013.

\bibitem{blu_surelet_deconv}
F. Xue, F. Luisier, and T. Blu, ``Multi-Wiener SURE-LET deconvolution," \emph{IEEE Trans. Image Process.}, vol. 22, no. 5, pp. 1954-1968, 2013.

\bibitem{newsure}
F. Luisier, T. Blu, and M. Unser, ``A new SURE approach to image denoising: Inter-scale orthonormal wavelet thresholding,''
\emph{IEEE Trans. Image Process.} vol. 16, no. 3, pp. 593--606, Mar. 2007.

\bibitem{blu_surelet_tip_2008}
F. Luisier and T. Blu, ``SURE-LET multichannel image denoising: interscale orthonormal wavelet thresholding," \emph{IEEE Trans. Image Process.}, vol. 17, no. 4, pp. 482--492, 2008.

\bibitem{nesterov_momentum1}
Y. E. Nesterov, \emph{Introductory Lectures on Convex Optimization: A Basic Course}, Kluwer Academic Publishers, London, 2004.

\bibitem{pearlmutter1994fast}
B.~A. Pearlmutter, ``Fast exact multiplication by the Hessian,'' \emph{Neural Computation}, vol.~6, no.~1, pp. 147--160, 1994.


\bibitem{fletcher_book}
R. Fletcher, \emph{Practical Methods of Optimization}. $2^{\text{nd}}$ Edition, John Wiley \& Sons, 1987.

%------------------------------------------------------------
%Online RLS references
\bibitem{malioutov_seq_cs_icassp}
D. M. Malioutov, S. Sanghavi, and A. S. Willsky, ``Compressed sensing with sequential observations," in \emph{Proc. IEEE Intl. Conf. on Acoustics, Speech and Signal Process.}, pp. 3357--3360, May 2008.

\bibitem{malioutov_seq_cs}
D. M. Malioutov, S. Sanghavi, and A. S. Willsky, ``Sequential compressed sensing," \emph{arXiv:1003.0219v1}, Mar. 2010. 

\bibitem{asif_romberg}
M. A. Asif and J. Romberg, ``Dynamic updating for $\ell_1$ minimization," \emph{IEEE J. Sel. Topics in Signal Process.}, vol. 4, no.2, pp. 421-434, Apr. 2010.

\bibitem{homotopy1}
P. J. Garrigues and L. E. Ghaoui, ``An homotopy algorithm for the Lasso with online observations," \emph{Adv. in Neural Info. Process. Systems (NIPS)}, pp. 489--496, 2009.

\bibitem{homotopy2}
A. Hofleitner, T. Rabbani, L. E. Ghaoui, and A. Bayen, ``Online homotopy algorithm for a generalization of the LASSO," \emph{IEEE Trans. Automatic Control}, vol. 58, no. 12, pp. 3175-3179, Apr. 2013.

\bibitem{twl}
D. Angelosante, J. A. Bazerque, and G. B. Giannakis, ``Online adaptive estimation of sparse signals: Where RLS meets the $\ell_1$-norm," \emph{IEEE Trans. Signal Process.}, vol. 58, no. 7, pp. 3436--3447, Jul. 2007.

\bibitem{kfcs1}
N. Vaswani, ``Analyzing least squares and Kalman filtered compressed sensing," in \emph{Proc. IEEE Intl. Conf. on Acoustics, Speech and Signal Process.}, pp. 3013--3016, Apr. 2009.

\bibitem{kfcs2}
C. Qiu, W. Lu, and N. Vaswani, ``Real-time dynamic MR image reconstruction using Kalman filtered compressed sensing," in \emph{Proc. IEEE Intl. Conf. on Acoustics, Speech and Signal Process.}, pp. 393--396, Apr. 2009.

\bibitem{distilled_sense1}
J. Haupt, R. Castro, and R. Nowak, ``Distilled sensing: Adaptive sampling for sparse detection and estimation," \emph{IEEE Trans. Info. Theory}, vol. 57, no. 9, pp. 6222--6235, 2011.

\bibitem{distilled_sense2}
J. Haupt, R. Baraniuk, R. Castro, and R. Nowak, ``Sequentially designed compressed sensing," in \emph{Proc. Statistical Signal Process. Workshop}, pp. 401--404, Oct. 2012.

\bibitem{takhar_csim}
D. Takhar, J. N. Laska, M. B. Wakin, M. F. Duarte, D. Baron, S. Sarvotham, K. F. Kelly, and R. G. Baraniuk, ``A new compressive imaging camera architecture using optical-domain compression," in \emph{Proc. SPIE, Computational Imaging IV}, Feb. 2006.


\bibitem{romberg_imaging}
J. Romberg, ``Imaging via compressive sampling," \emph{IEEE Signal Process. Mag.}, vol. 25, no. 2, pp. 14--20, Mar. 2008.

\bibitem{willett}
R. M. Willett, R. F. Marcia, and J. M. Nichols, ``Compressed sensing for practical optical imaging systems: A tutorial," \emph{Optical Engg.}, vol. 50, no. 7, Jul. 2011.

\bibitem{spc}
M. F. Duarte, M. A. Davenport, D. Takhar, J. N. Laska, T. Sun, K. F. Kelly, and R. G. Baraniuk, ``Single-pixel imaging via compressive sampling," \emph{IEEE Signal Process. Mag.}, vol. 25, no. 2, pp. 83--91, Mar. 2008.

\bibitem{csim_color}
P. Nagesh and B. Li, ``Compressive imaging of color images," in \emph{Proc. IEEE Intl. Conf. on Acoustics, Speech and Signal Process.}, pp.  1261--1264, Apr. 2009.

\bibitem{fpa_cs_rice}
H. Chen, M. S. Asif, A. C. Sankaranarayanan, and A. Veeraraghavan, ``FPA-CS: Focal plane array-based compressive imaging in short-wave infrared," in \emph{Proc. Computer Vision and Pattern Recognition}, pp. 2358--2366, 2015.

%------------------------------------------------------------
%Sparse Fienup references
\bibitem{crystallography_chspr}
R. P. Millane, ``Phase retrieval in crystallography and optics," \emph{J. Opt. Soc. Amer. A}, vol. 7, no. 3, pp. 394--411, Mar. 1990.

\bibitem{holography_chspr}
 A. Szoke, ``Holographic microscopy with a complicated reference," \emph{J. Imag. Sci. Technol.}, vol. 41, pp. 332--341, 1997.
 
\bibitem{microscopy_chspr} 
A. J. J. Drenth, A. Huiser, and H. Ferwerda, ``The problem of phase retrieval in light and electron microscopy of strong objects," \emph{Optica Acta}, vol. 22, pp. 615--628, 1975.

\bibitem{fienup_main1}
J. R. Fienup, ``Phase retrieval algorithms: A comparison," \emph{Appl. Opt.}, vol. 21, pp. 2758--2769, 1982.

\bibitem{fienup_main2}
J. R. Fienup, ``Phase retrieval algorithms: A personal tour [invited]," \emph{Appl. Opt.}, vol. 52, pp. 45--56, 2013.

\bibitem{gs_pr}
R. W. Gerchberg and W. O. Saxton, ``A practical algorithm for the determination of phase from image and diffraction plane pictures," \emph{Optik}, vol. 35, pp. 237--246, 1972.

\bibitem{bauschke_pr}
H. H. Bauschke, P. L. Combettes, and D. Luke, ``Phase retrieval, error reduction algorithm, and Fienup variants: A view from convex optimization," \emph{J. Opt. Soc. Amer. A}, vol. 19, pp. 1334--1345, 2002.

\bibitem{quatieri_pr}
T. F. Quatieri and A. V. Oppenheim, ``Iterative techniques for minimum-phase signal reconstruction from phase or magnitude," \emph{IEEE Trans. Acoust., Speech, Signal Process.}, vol. 29, pp. 1187--1193, 1981.

\bibitem{yegna_pr}
B.Yegnanarayana and A. Dhayalan, ``Noniterative techniques for minimum phase signal reconstruction from phase or magnitude," in \emph{Proc. IEEE Intl. Conf. Acoust., Speech, and Signal Process.}, vol. 8, pp. 639--642, Apr. 1983.

\bibitem{css_holography}
C. S. Seelamantula, N. Pavillon, C. Depeursinge, and M. Unser, ``Exact complex-wave reconstruction in digital holography," \emph{J. Opt. Soc. Amer. A}, vol. 28, no. 6, pp. 983--992, Jun. 2011.

\bibitem{param2D_icip}
B. A. Shenoy, S. Mukherjee, and C. S. Seelamantula, ``Phase retrieval for a class of 2-D signals characterized by first-order difference equations," in \emph{Proc. IEEE Intl. Conf. on Image Process.}, pp. 325--329, 2013.

\bibitem{param2D_tip}
B. A. Shenoy and C. S. Seelamantula, ``Exact phase retrieval for a class of 2-D parametric signals," \emph{IEEE Trans. Signal Process.}, vol. 63, no. 1, pp. 90--103, 2015.

\bibitem{pr_shift_invar}
B. A. Shenoy, S. Mulleti, and C. S. Seelamantula, ``Exact phase retrieval in principal shift-invariant spaces," \emph{IEEE Trans. Signal Process.}, vol. 64, no. 2, pp. 406--416, 2016.

\bibitem{moravec_cpr}
M. L. Moravec, J. K. Romberg, and R. G. Baraniuk, ``Compressive phase retrieval," in \emph{Proc. Wavelets XII SPIE Int. Symp. Opt. Sci. Technol.}, Aug. 2007.

\bibitem{yu_vettreli_ssf}
Y. M. Yu and M. Vetterli, ``Sparse spectral factorization: Unicity and reconstruction algorithms," in \emph{Proc. IEEE Intl. Conf. Acoust. Speech, Signal Process.}, pp. 5976--5979, 2011.

\bibitem{gespar}
Y. Shechtman, A. Beck, and Y. C. Eldar, ``GESPAR: Efficient phase retrieval of sparse signals," \emph{IEEE Trans. Signal Process.}, vol. 62, no. 4, pp. 928--938, Feb. 2014. 

\bibitem{netrapalli_altminpr}
P. Netrapalli, P. Jain, and S. Sanghavi, ``Phase retrieval using alternating minimization," \emph{IEEE Trans. Signal Process.}, vol. 63, no. 18, pp. 4814--4826, Sep. 2015.

\bibitem{low_rank_PR_vaswani}
N. Vaswani, S. Nayer, and Y. C. Eldar, ``Low rank phase retrieval," \emph{IEEE Trans. Signal Process.}, vol. 65, no. 15, pp. 4059--4074, Aug. 2017.

\bibitem{dolphin}
A. M. Tillmann, Y. C. Eldar, and J. Mairal, ``DOLPHIn--Dictionary learning for phase retrieval," \emph{IEEE Trans. Signal Process.}, vol. 64, no.
24, pp. 6485--6500, Dec. 2016.

\bibitem{tfocs}
S. Becker, E. J. Cand\`es, and M. Grant, ``Templates for convex cone problems with applications to sparse signal recovery," \emph{Technical Report}, Department of Statistics, Stanford University, 2010.

\bibitem{schniter_gamp}
P. Schniter and S. Rangan, ``Compressive phase retrieval via generalized approximate massage passing," \emph{IEEE Trans. Signal Process.}, vol. 63, no. 4, pp. 1043--1055, Feb. 2015.

\bibitem{bspr_peng}
W. Peng and H. Wang, ``Binary sparse phase retrieval via simulated annealing," \emph{Math. Probl. in Engg.}, Article ID 8257612, May 2016.

\bibitem{palomar_mm}
T. Qiu and D. P. Palomar, ``Undersampled sparse phase retrieval via majorization-minimization," \emph{IEEE Trans. Signal Process.}, vol. 65, no. 22, pp. 5957--5969, Nov. 2017.

\bibitem{fogel_pr_imaging}
F. Fogel, I. Waldspurger, and A. d'Aspremont, ``Phase retrieval for imaging problems," \emph{arXiv:1304.7735v2}, Apr. 2014.

\bibitem{PL1_candes}
E. J. Cand\`es, T. Strohmer, and V. Voroninski, ``PhaseLift: Exact and stable signal recovery from magnitude measurements via convex programming," \emph{Comm. Pure and Appl. Math.}, vol. 66, issue 8, pp. 1241--1274, Aug. 2013.

\bibitem{PL2_candes}
E. J. Cand\`es, Y. C. Eldar, T. Strohmer, and V. Voroninski, ``Phase retrieval via matrix completion," \emph{SIAM J. Imag. Sci.}, vol. 6, issue 1, pp. 199--224, Feb. 2013.  

\bibitem{cpr_pl}
H. Ohlsson, A. Y. Yang, R. Dong, and S. S. Sastry, ``Compressive phase retrieval from squared output measurements via semidefinite programming," \emph{arXiv:1111.6323v3}, Mar. 2012.

\bibitem{qcs_eldar}
Y. Shechtman, Y. C. Eldar, A. Szameit, and M. Segev, ``Sparsity based sub-wavelength imaging with partially incoherent light via quadratic compressed sensing," \emph{Opt. Exp.}, vol. 19, no. 16, pp. 14807--14822, 2011.

\bibitem{power_it}
G. H. Golub and C. H. Van Loan, \emph{Matrix Computations}. $4^{\text{th}}$ Edition, JHU Press, Oct. 1996.

\bibitem{candes_wf_it}
E. J. Cand\`es, X. Li, and M. Soltanolkotabi, ``Phase retrieval via Wirtinger flow: Theory and algorithms," \emph{IEEE Trans. Info. Theory}, vol. 61, no. 4, pp. 1985--2007, Apr. 2015.

\bibitem{candes_twf}
Y. Chen and E. J. Cand\`es, ``Solving random quadratic systems of equations is nearly as easy as solving linear systems," in \emph{Proc. Adv. in Neural Info. Process. Systems (NIPS)}, 2015. 

\bibitem{phasecut}
I. Waldspurger, A. dÕAspremont, and S. Mallat, ``Phase recovery, max-cut and complex semidefinite
programming," \emph{Math. Program.}, vol. 149, no. 1, pp. 47--81, 2015.

\bibitem {luke_pr_diff_image}
D.~R.~Luke, ``Relaxed averaged alternating reflections for diffraction imaging," {\it Inverse Problems}, vol.~21, pp.~37--50, 2005.

\bibitem{oppenheim_dsp_book}
A. V. Oppenheim, R. W. Schaffer, and J. R. Buck, \emph{Discrete-Time Signal Processing}. Prentice Hall, 1998. 

\bibitem{css_oct_2008} 
C.~S.~Seelamantula, M.~L.~Villiger, R.~A.~Leitgeb, and M.~Unser, ``Exact and efficient signal reconstruction in frequency-domain optical coherence tomography," \emph{J. Opt. Soc. Am. (A),} vol.~25, no.~7, pp.~1762--1771, Jul.~2008.

\bibitem{ozcan_oct_2006}
A. Ozcan, M. J. F. Digonnet, and G. S. Kino, ``Minimum-phase-function-based processing in frequency-domain optical-coherence tomography systems," \emph{J. Opt. Soc. Am. A}, vol. 23, pp. 1669--1677, 2006.

\bibitem{css_iisc_journal}
C. S. Seelamantula and T. Lasser, ``Hilbert transform relations in frequency-domain optical-coherence
tomographic imaging," Invited article, \emph{J. Indian Institute of Science, Special issue on Imaging and Microscopy}, vol. 93, no. 1, pp. 139--148, Mar. 2013.

\bibitem{morgan_colormap} 
M. Geissbuehler and T. Lasser, ``How to display data by color schemes compatible with red-green color perception deficiencies,'' \emph{Optics Express}, vol. 21, pp. 9862--9874, 2013.



%-----------QPR references
\bibitem{zymnis_qcs}
A. Zymnis, S. Boyd, and E. J. Cand\`es, ``Compressed sensing with quantized measurements," \emph{IEEE Signal Process. Lett.}, vol. 17, no. 2, pp. 149--152, Feb. 2010. 

\bibitem{laska1}
J. Laska, P. Boufounos, M. Davenport, and R. Baraniuk, ``Democracy in action: Quantization, saturation, and compressive sensing," \emph{Applied and Computational Harmonic Analysis}, vol. 31(3), pp. 429--443, Nov. 2011.

\bibitem{qcs_bit_precision}
E. Ardestanizadeh, M. Cheraghchi, and A. Shokrollahi, ``Bit precision analysis for compressed sensing," in \emph{Proc. IEEE Intl. Symp. on Info. Theory}, pp. 1--5, 2009.

\bibitem{binary_imaging1}
A Bourquard, F. Aguet, and M. Unser, ``Optical imaging using binary sensors," \emph{Opt. Exp.}, vol. 18, no. 5, Mar. 2010.

\bibitem{binary_imaging2}
A Bourquard and M. Unser, ``Binary compressed imaging," \emph{IEEE Trans. Image Process.}, vol. 22, no. 3, pp. 1042--1055, Mar. 2013.

\bibitem{baraniuk1}
P. T. Boufounos and R. G. Baraniuk, ``1-bit compressive sensing," in \emph{Proc. Conf. Info. Science and Systems}, Princeton, NJ, Mar. 2008.

\bibitem{plan1}
Y. Plan and R. Vershynin, ``One-bit compressed sensing by linear programming," \emph{arXiv:1109.4299v5}, Mar. 2012.

\bibitem{msp}
P. T. Boufounos, ``Greedy sparse signal reconstruction from sign measurements," in \emph{Proc. Asilomar Conf.  Signals, Systems, and Computation}, Asilomar, CA, Nov. 2009.

\bibitem{var_gamma_ref}
D.B. Madan and E. Seneta, ``The variance gamma (V.G.) model for share market returns," \emph{J. Business}, vol. 63, no. 4, pp. 511--524, Oct. 1990.

\bibitem{jayant_noll}
N. S. Jayant and P. Noll, \textit{Digital Coding of Waveforms: Principles and Applications to Speech and Video}. Prentice-Hall, USA, 1984.

\bibitem{bstj_paper}
B. Smith, ``Instantaneous companding of quantized signals," \emph{Bell System Tech. J.}, vol. 36, pp. 653--709, May 1957.


\bibitem{svt_candes}
J.-F. Cai, E. J. Cand\`es, and Z. Shen, ``A singular value thresholding algorithm for matrix completion," \emph{SIAM J. Optimization}, vol. 20, no. 4, pp. 1956--1982, Mar. 2010.


\bibitem{geng_yang}
J. Geng, X. Yang, X. Wang, and L. Wang, ``An accelerated iterative hard-thresholding method for matrix completion," \emph{Intl. J. Signal Process., Image Process., and Pattern Recog.}, vol. 8, no. 7, pp. 141--150, 2015.

\bibitem{balan1_qpr}
R. Balan, ``Reconstruction of signals from magnitudes of redundant representations: The complex case," \emph{Found. Comp. Math.}, pp. 1--45, 2013.
 
\bibitem{balan2_qpr}
R. Balan, ``The Fisher information matrix and the CRLB in a non-AWGN model for the phase retrieval problem," in \emph{Proc. Intl. Conf. Sampl. Theory and Applications}, pp. 178--182, 2015. 

\bibitem{pr_crb_fpp_qpr}
C. Qian, N. D. Sidiropoulos, K. Huang, L. Huang, and H. C. So, ``Phase retrieval using feasible point pursuit: Algorithms and Cram\'er-Rao bound," \emph{IEEE Trans. Signal Process.}, vol. 64, no. 20, pp. 5282--5296, Oct. 2016.

\bibitem{bandeira_qpr}
 A. S. Bandeira, J. Cahill, D. G. Mixon, and A. A. Nelson, ``Saving phase: Injectivity and stability for phase retrieval," \emph{Appl. and Comp. Harmonic Anal.}, vol. 37, no. 1, pp. 106--125, 2014.

\bibitem{cederquist_qpr}
J. N. Cederquist and C. C. Wackerman, ``Phase-retrieval error: A lower bound," \emph{J. Opt. Soc. Amer. A}, vol. 4, no. 9, pp. 1788--1792, 1987.


\end{thebibliography}


==> bibliography_thesis.tex <==
\begin{thebibliography}{999}
\newcommand{\enquote}[1]{``#1''}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\noopsort}[1]{}
\providecommand{\switchargs}[2]{#2#1}

%\bibitem{CIPIC}
%V. R. Algazi, R. O. Duda, D. M. Thompson and C. Avendano,
%\newblock  ``The CIPIC HRTF database,"
%\newblock in \emph{Proc. IEEE Workshop Appl. Sig. Proc. to Audio and Acoust.}, pp. 99--102, 2001.

%%%----------------------------------------
%Intro references
\bibitem{hvpoor_book}
H. V. Poor, \emph{An Introduction to Signal Detection and Estimation}., $2^{\text{nd}}$ Edition, Spronger-Verlang, 1994.


\bibitem{landweber}
L. Landweber, ``An iteration formula for Fredholm integral equations of the first kind," \emph{Amer. J. Math.}, vol. 73, pp. 615--624, 1951.

\bibitem{nonlin_landweber}
M. Hanke, A. Neubauer, and O. Scherzer, ``A convergence analysis of the Landweber iteration for nonlinear ill-posed problems," \emph{Numerische Mathematik}, Vol. 72, no. 1, pp. 21--37, 1995.

\bibitem{landweber_thesis}
T. Nikazad, ``The use of Landweber algorithm in image reconstruction," \emph{Link\"oping Studies in Sci. and Tech.}, Thesis no. 1311 (Link\"oping Universitet, Sweden), 2007. 

\bibitem{semi_conv_hansen}
T. Elfving, T. Nikazad, and P. C. Hansen, ``Semi-Convergence and Relaxation Parameters for a class of SIRT algorithms," \emph{Electronic Trans. Numerical Analysis}. vol. 37, pp. 321--336, 2010.


\bibitem{tikhonov_book1}
A. N. Tikhonov, A. V. Goncharsky, V. V. Stepanov, and A. G. Yagola, \emph{Numerical Methods for the Solution of Ill-Posed Problems.} Kluwer Academic Publishers, 1995.

\bibitem{tikhonov_book2}
A. N. Tikhonov, A. S. Leonov, A. G. Yagola, \emph{Nonlinear Ill-Posed Problems.} Chapman and Hall, 1998.


\bibitem{tv_reg_ref}
D. Strong and T.Chan, ``Edge-preserving and scale-dependent properties of total variation regularization," \emph{Inverse Problems}, vol. 19, pp. 165--187, 2003.

\bibitem{jain_iht}
P. Jain, A. Tewari, and P. Kar, ``On iterative hard thresholding methods for high-dimensional M-estimation," in \emph{Proc. Adv. in Neural Info. Process. Systems (NIPS)}, pp. 685--693, 2014. 

\bibitem{parikh_boyd_admm}
S. Boyd, N. Parikh, E. Chu, B. Peleato, and J. Eckstein, ``Distributed optimization and statistical learning via the alternating direction method of multipliers," 
\emph{Foundations and Trends in Mach. Learn.}, vol. 3, no. 1, pp. 1--122, 2011.

\bibitem{prox_grad_beck}
A. Beck and M. Teboulle, ``Gradient-based algorithms with applications to signal recovery problems," in \emph{Convex Optimization in Signal Process. and Comm.}, (D. Palomar and Y. Eldar, eds.), pp. 42--88, Cambridge University Press, 2010.

\bibitem{omp_guarantee}
J. Wang and B. Shim, ``On the recovery limit of sparse signals using orthogonal matching pursuit," \emph{IEEE Trans. Signal Process.},  vol. 60, no. 9, pp. 4973--4976, Sep. 2012. 


\bibitem{blumensath_iht}
T. Blumensath and M. E. Davies, ``Iterative hard thresholding for compressed sensing," \emph{Appl. Comput. Harmon. Anal.}, vol. 27, issue 3, pp. 265--274, 2009.

\bibitem{ds_annala_stat}
E. J. Cand\`es and T. Tao, ``The Dantzig Selector: Statistical estimation when $p$ is much larger than $n$," \emph{The Annals of Stat.}, vol. 35, no. 6, pp. 2313--2351, 2007.
%%%----------------------------------------
%Robust DL references
\bibitem{candes_cs_intro_2008}
E. J.~Cand\`es and M.~Wakin, ``An introduction to compressive sampling,'' {\em IEEE Signal Process. Mag.}, vol.~25, pp.~21 --30, Mar. 2008.

\bibitem{baraniuk_cs_tutorial}
R. Baraniuk, ``Compressive sensing," \emph{IEEE Signal Process. Mag.}, vol. 24, no. 4, pp. 118--121, Jul. 2007.

\bibitem{candes_tao_org}
E. J. Cand\`es, J. Romberg, and T. Tao, ``Robust uncertainty principles: Exact signal reconstruction from highly incomplete frequency information," \emph{IEEE Trans. Info. Theory,} vol. 52, no. 2, pp. 489--509, Feb. 2006.

\bibitem{donoho_it}
D. Donoho, ``Compressed sensing," \emph{IEEE Trans. Info. Theory}, vol. 52, no. 4, pp. 1289--1306, Apr. 2006.

\bibitem{elad_book}
M. Elad, \emph{Sparse and Redundant Representations: From Theory to Applications in Signal and Image Processing}. Springer, 2010.

\bibitem{rubinstein_dl_review}
R. Rubinstein, A. M. Bruckstein, and M. Elad, ``Dictionaries for sparse representation modeling," \emph{Proc. IEEE}, vol. 98, no. 6, pp. 1045--1057, Jun. 2010.

\bibitem{tosic_dl_review}
I. Tosic and P. Frossard, ``Dictionary learning," \emph{IEEE Signal Process. Mag.}, vol. 28, no. 2, pp. 27--38, Mar. 2011.

\bibitem{elad_ksvd_tip}
M. Elad and M. Aharon, ``Image denoising via sparse and redundant representations over learned dictionaries," \emph{IEEE Trans. Image Process.}, vol. 15, no. 12, pp. 3736--3745, Dec. 2006.

\bibitem{elad_ksvd_tsp}
M. Aharon, M. Elad, and A. Bruckstein, ``K-SVD: An algorithm for designing overcomplete dictionaries for sparse representation," \emph{IEEE Trans. Signal Process.}, vol. 54, no. 11, pp. 4311--4322, Nov. 2006.

\bibitem{arora_ksvd}
S. Arora, R. Ge, and A. Moitra, ``New algorithms for learning incoherent and over-complete dictionaries," \emph{J. Mach. Learn. Res.}, vol. 35, pp. 1--28, 2014. 

\bibitem{schnass_ksvd}
K. Schnass, ``On the identifiability of over-complete dictionaries via the minimization principle underlying K-SVD," \emph{Appl. and Comp. Harmonic Anal.}, vol. 37, issue 3, pp. 464--491, Nov. 2014. 

\bibitem{dai_simco}
W. Dai, T. Xu, and W. Wang, ``Simultaneous codeword optimization (SimCO) for dictionary update and learning," \emph{IEEE Trans. Signal Process.}, vol. 60, no. 12, pp. 6340--6353, Dec. 2012.

\bibitem{engan_mod}
K. Engan, S. O. Aase, and J. H. Husoy, ``Method of optimal directions for frame design," \emph{in   Proc. IEEE Intl. Conf. on Accoust., Speech, and Signal Process.}, pp. 2443--2446, Mar. 1999. 

\bibitem{yang_sr}
J. Yang, J. Wright, T. S. Huang, and Y. Ma, ``Image super-resolution via sparse representation," \emph{IEEE Trans. Image Process.}, vol. 19, no. 11, pp. 2861--2873, Nov. 2010.

\bibitem{sujit_inp}
S. Sahoo and W. Lu, ``Image in-painting using sparse approximation with adaptive window selection," in \emph{Proc. IEEE Intl. Symp. on Intell. Signal Process.}, pp. 1--4, Sep. 2011.

\bibitem{julien_imrest}
J. Mairal, M. Elad, and G. Sapiro, ``Sparse representation for color image restoration,"  \emph{IEEE Trans. Image Process.}, vol. 17, pp. 53--69, Jan. 2008.

\bibitem{zhang_cvpr}
Q. Zhang and B. Li, ``Discriminative K-SVD for dictionary learning in face recognition," in \emph{Proc. Conf. on Comp. Vis. and Pattern Recog.  (CVPR)}, pp. 2691--2698, 2010.

\bibitem{jiang_cvpr}
Z. Jiang, Z. Lin, and L. S. Davis, ``Learning a discriminative dictionary for sparse coding via label consistent K-SVD," in Proc. \emph{Proc. Conf. on Comp. Vis. and Pattern Recog.  (CVPR)}, pp. 1697--1704, 2011.

\bibitem{dtao_multiview_hessian}
W. Liu, D. Tao, J. Cheng, and Yuanyan Tang, ``Multiview Hessian discriminative sparse coding for image annotation," \emph{Elsevier Computer Vision and Image Understanding}, vol. 118, pp. 50--60, Jan. 2014.

\bibitem{dtao_group_sparse}
Y. Sun, Q. Liu, J. Tang, and D. Tao, ``Learning discriminative dictionary for group sparse representation," \emph{IEEE Trans. Image Process.}, vol. 23, no. 9, pp. 3816--3828, Sep. 2014.

\bibitem{liangyueli_elsevier}
L. Li, S. Li, and Y. Fu, ``Learning low-rank and discriminative dictionary for image classification," \emph{Elsevier Signal Process.}, vol. 32, no. 10, pp. 814--823, Oct. 2014.

\bibitem{yangfeixu_elsevier} 
Y. Xu, G. Bao, X. Xu, and Z. Ye, ``Single-channel speech separation using sequential discriminative dictionary learning," \emph{Elsevier Signal Process.}, vol. 106, pp. 134--140, Jan. 2015.

\bibitem{vahid_abolghasemi} 
V. Abolghasemi and S. Ferdowsi, ``EEGÐfMRI: Dictionary learning for removal of ballistocardiogram artifact from EEG," \emph{Elsevier Biomedical Signal Process. and Control}, vol. 18, pp. 186--194, Apr. 2015.


\bibitem{zgao_elsevier}
Z. Gao, H. Zhang, G. P. Xu, Y. B. Xue, and A. G. Hauptmann, ``Multi-view discriminative and structured dictionary learning with group sparsity for human action recognition," \emph{Elsevier Signal Process.}, vol. 112, pp. 83--97, Jul. 2015.

\bibitem{bishop_prml_book}
C.~M.~Bishop, \emph{Pattern Recognition and Machine Learning}. Springer, 2006.

\bibitem{dtao_geometric_mean}
D. Tao, X. Li, X. Wu, and S. J. Maybank, ``Geometric mean for subspace selection," \emph{IEEE Trans. Pattern Anal. Mach. Intell.}, vol. 31, no. 2, pp. 260--274, Feb. 2009.

\bibitem{kasiviswanathan_nips} 
S. P. Kasiviswanathan, H. Wang, A. Banerjee, and P. Melville, ``Online $\ell_1$ dictionary learning with application to novel document detection," in \emph{Proc. Adv. in Neural Info. Proc. Systems (NIPS)}, vol. 25, pp. 2267--2275, 2012.

\bibitem{spk_icassp}
S. P. Kasiviswanathan, ``Fast online $\ell_1$ dictionary learning algorithm for novel document detection," in \emph{Proc. IEEE Intl. Conf. on Accoust., Speech, and Signal Process.}, pp. 8585--8589, 2013.

\bibitem{tao_manhattan}
T. Liu and D. Tao, ``On the performance of Manhattan nonnegative matrix factorization," \emph{IEEE Trans. on Neural Networks and Learning Systems}, issue 99, Aug. 2015. 

\bibitem{lu_rdl}
C. Lu, J. Shi, and J. Jia, ``Online robust dictionary learning," in Proc. \emph{IEEE Conf. on Comp. Vis. and Patt. Recog.}, pp. 415--422, 2013.

\bibitem{online_DL}
J. Mairal, F. Bach, J. Ponce, and G. Sapiro, ``Online dictionary learning for sparse coding," in \emph{Proc. $26^{\text{th}}$ Annual Intl. Conf. on Machine Learning}, pp. 689--696, 2009.

\bibitem{wang_elsev}
S. Wang, Q. Liu, Y. Xia, P. Dong, J. Luo, Q. Huang, and D. D. Feng, ``Dictionary learning based impulse noise removal via $\ell_1-\ell_1$ minimization," \emph{Elsevier Signal Process.}, vol. 93, no. 9, pp. 2696--2708, Sep. 2013.  


\bibitem{tao_cauchy}
T. Liu and D. Tao, ``On the robustness and generalization of Cauchy regression," in Proc. \emph{IEEE Intl. Conf. on Information Science and Technology} (ICIST), pp. 100--105, Apr. 2014.  

\bibitem{daubechies_irls} 
I. Daubechies, R. DeVore, M. Fornasier, and C. S. G\"{u}nt\"{u}rk, ``Iteratively re-weighted least-squares minimization for sparse recovery," \emph{Comm. Pure and Appl. Math.}, vol. LXIII, pp. 1--38, 2010.


\bibitem {miosso_irls} 
C. J. Miosso, R. V. Borries, M. Arg\'{a}ez, L. Velazquez, C. Quintero, and C. M. Potes, ``Compressive sensing reconstruction with prior information by iteratively reweighted least-squares," \emph{IEEE Trans. Signal Process.}, vol. 57, no. 6, pp. 2424--2431, Jun. 2009.

\bibitem{endra_irls}
O. Endra and Gunawan, ``Comparison of $\ell_1$-minimization and iteratively reweighted least-squares-$\ell_p$-minimization for image reconstruction from compressive sensing," in \emph{Proc. Second Intl. Conf. on Advances in Computing, Control and Telecom. Tech.}, pp. 85--88, Dec. 2010.

\bibitem{tao_label_noise}
T. Liu and D. Tao, ``Classification with noisy labels by importance reweighting," \emph{IEEE Trans. Pattern Anal. and Mach. Intell.}, vol. 38, no. 3, pp. 447--461, Jul. 2015. 

\bibitem{grant_cvx} 
M. Grant and S. Boyd, ``CVX: Matlab software for disciplined convex programming," version 2.0 beta, Sep. 2013.


\bibitem{manopt}
N. Boumal, B. Mishra, P. A. Absil, and R. Sepulchre, ``ManOpt, a MATLAB toolbox for optimization on manifolds," \emph{J. Mach. Learning Res.}, vol. 15, pp. 1455--1459, 2014. 

\bibitem{brian_jeffs}
B. D. Jeffs and M. Gunsay, ``Restoration of blurred star field images by maximally sparse optimization," \emph{IEEE Trans. Image Process.}, vol. 2, no. 2, pp. 202--211, Apr. 1993.

\bibitem{ssim_paper_ref}
Z. Wang, A. C. Bovik, H. R. Sheikh, and E. P. Simoncelli, ``Image quality assessment: From error visibility to structural similarity," \emph{IEEE Trans. Image Process.}, vol. 13, no. 4, pp. 600--612, Apr. 2004.

\bibitem{bartlett_jmlr}
P. L. Bartlett and S. Mendelson, ``Rademacher and Gaussian complexities: Risk bounds and structural results," \emph{J. Mach. Learning Res.}, vol. 3, pp. 463--482, 2002.  

\bibitem{sudakov_ineq1}
V. N. Sudakov, ``Gaussian random processes and measures of solid angles in Hilbert space," \emph{Dokl. Akad. Nauk. SSR} vol. 197, pp. 412--415, 1971.

\bibitem{sudakov_ineq_proof}
S. Chatterjee, ``An error bound in the Sudakov-Fernique inequality," \emph{arXiv:math/0510424v1} Oct. 2005.

\bibitem{vahid}
V. Abolghasemi, S. Ferdowsi, and S. Sanei, ``Blind separation of image sources via adaptive dictionary learning," \emph{IEEE Trans. Image Process.}, vol. 21, no. 6, pp. 2921--2930, Jun. 2012.

\bibitem{SPK_nips}
S. P. Kasiviswanathan, H. Wang, A. Banerjee, and P. Melville, ``Online $\ell_1$-dictionary learning with application to novel document detection," in  \emph{Proc. Adv. in Neural Info. Proc. Systems (NIPS)}, vol. 3, pp. 2258--2266, 2012. 


\bibitem{bao}
C. Bao, J. Cai, and H. Ji, ``Fast sparsity-based orthogonal dictionary learning for image restoration," in \emph{Proc. IEEE Intl. Conf. on Comp. Vis.}, pp. 3384--3391, 2013.


%--------------------------------------
%DCDL references
\bibitem{rubinstein_double_sparsity}
R. Rubinstein, M. Zibulevsky, and M. Elad, ``Double sparsity: Learning sparse dictionaries for sparse signal approximation," \emph{IEEE Trans. Signal Process.}, vol. 58, no. 3, pp. 1553--1564, Mar. 2010.

\bibitem{naai}
N. Ai, J. Peng, X. Zhu, and X. Feng, ``SISR via trained double sparsity dictionaries," \emph{Multimedia Tools and Applications}, vol. 74, issue 6, pp. 1997--2007, Mar. 2015. 


\bibitem{online_DL_JMLR}
J. Mairal, F. Bach, J. Ponce, and G. Sapiro, ``Online learning for matrix factorization and sparse coding," \emph{J. Mach. Learn. Res.}, vol. 11, pp. 19--60, 2010.

\bibitem{cherian}
A. Cherian, S. Sra, and N. Papanikolopoulos, ``Denoising sparse noise via online dictionary learning," \emph{in Proc. IEEE Intl. Conf. on Accoust., Speech, and Signal Process.}, pp. 2060--2063, May 2011.

\bibitem{mackey}
L. Mackey, A. Talwalkar, and M. I. Jordan, ``Distributed matrix completion and robust factorization," \emph{J. Mach. Learn. Res.}, vol. 16, pp. 913--960, 2015.

\bibitem{chainais}
P. Chainais and C. Richard, ``Distributed dictionary learning over a sensor network," \emph{arXiv:1304.3568v1}, Apr. 2013.

\bibitem{liang_dist}
J. Liang, M. Zhang, X. Zeng, and G. Yu, ``Distributed dictionary learning for sparse representation is sensor networks," \emph{IEEE Trans. Image Process.}, vol. 23, no. 6, pp. 2528--2541, Jun. 2014.

\bibitem{dai_cluster}
T. Xu, W. Dai, and W. Wang, ``Fast dictionary learning algorithm via codeword clustering and hierarchical sparse coding," in \emph{Proc. $9^{\text{th}}$ IMA Intl. Conf. on Math. in Signal Process.}, Dec. 2012.

\bibitem{cormen_algo}
T. H. Cormen, C. E. Leiserson, R. L. Rivest, and C. Stein, \emph{Introduction to Algorithms $3^{\text{rd}}$ Edition}, The MIT Press, 2005.

\bibitem{tropp_omp}
J. A. Tropp and A. C. Gilbert, ``Signal recovery from random measurements via orthogonal matching pursuit," \emph{IEEE Trans. Info. Theory}, vol. 53, no. 12, pp. 4655--4666, Dec. 2007.


%------------------------------------------------------------
%SVR references
\bibitem{tropp_cosamp}
D.Needell and J.A.Tropp, ``CoSaMP: Iterative signal recovery from incomplete and inaccurate samples," \emph{Appl. and Comp. Harmonic Anal.}, vol. 26, issue 3, pp. 301--321, May 2009. 

\bibitem{donoho_bp_siam}
S. S. Chen, D. L. Donoho, and M. A. Saunders, ``Atomic decomposition by basis pursuit", \emph{SIAM J. of Sci. Comp.}, vol. 20, no. 1, pp. 33--61, Feb. 1997.


\bibitem{anal_ksvd1}
R. Rubinstein, T. Peleg, and M. Elad, ``Analysis K-SVD: A dictionary learning algorithm for the analysis sparse model," \emph{IEEE Trans. Signal Process.}, vol. 61, no. 3, pp. 661--677, Feb. 2013.

\bibitem{dai_analysis}
J. Dong, W. Wang, and W. Dai, ``Analysis SimCO: A new algorithm for analysis dictionary learning," in \emph{Proc. IEEE Intl. Conf. on Accoust., Speech, and Signal Process.}, pp. 7193--7197, May 2014.

\bibitem{ravishankar_TL1}
S. Ravishankar and Y. Bresler, ``Learning sparsifying transforms," \emph{IEEE Trans. Signal Process.}, vol. 61, no. 5, pp. 1072--1086, Mar. 2013.

\bibitem{ravishankar_TL2}
S. Ravishankar and Y. Bresler, ``$\ell_0$ sparsifying transform learning with efficient optimal updates and convergence guarantees," \emph{IEEE Trans. Signal Process.}, vol. 63, no. 9, pp. 2389--2404, May 2015.

\bibitem{ravishankar_online}
S. Ravishankar, B. Wen, and Y. Bresler, ``Online sparsifying transform learning--Part I: Algorithms," \emph{IEEE J. Selected Topics in Signal Process.}, vol. 9, no. 4, pp. 625--636, Jun. 2015.

\bibitem{transform_ksvd_ender}
E. M. Eksioglue and O. Bayir, ``K-SVD meets transform learning: Transform K-SVD," \emph{IEEE Signal Process. Lett.}, vol. 21, no. 3, pp. 347--351, Mar. 2014.

\bibitem{tight_frame_cai}
J.-F.  Cai, H. Ji, Z. Shen, and G.-B. Ye, ``Data-driven tight frame construction and image denoising," \emph{Appl. and Computational Harmonic Anal.}, vol. 37, issue 1, pp. 89-105, Jul. 2014. 

\bibitem{IPR_plumbley}
D. Barchiesi and M. D. Plumbley, ``Learning incoherent dictionaries for sparse approximation using iterative projections and rotations," \emph{IEEE Trans. Signal Process.}, vol. 61, no. 8, pp. 2055--2065, Apr. 2013.

\bibitem{opp_66}
P. H. Sch\"onemann, ``A generalized solution of the orthogonal Procrustes problem," \emph{Psychometrika}, vol. 31, issue 1, pp. 1--10, Mar. 1966.

\bibitem{ortho_sc}
H. Sch\"utze, E. Barth, and T. Martinetz, ``Learning efficient data representations with orthogonal sparse coding," \emph{IEEE Trans. Computational Imaging}, vol. 2, no. 3, pp.177--189, Sep. 2016.

\bibitem{bm3d_tip}
K. Dabov, A. Foi, V. Katkovnik, and K. Egiazarian, ``Image denoising by sparse 3D transform-domain collaborative filtering," \emph{IEEE Trans. Image Process.}, vol. 16, no. 8, pp. 2080--2095, 2007.


%------------------------------------------------------------
%LETnet/fLETnet references
\bibitem{candes_romberg_tao}
E. J. Cand\`es, J. Romberg, and T. Tao, ``Stable signal recovery from incomplete and inaccurate measurements," \emph{Comm. Pure and Appl. Math.} vol. 59 no. 8, pp. 1207--1223, 2006.

\bibitem{krizhevsky2012imagenet}
A. Krizhevsky, I. Sutskever, and G. E. Hinton, ``ImageNet classification
with deep convolutional neural networks," in \emph{Proc. Adv. in Neural Info. Process. Systems (NIPS)}, pp. 1097--1105, 2012.

\bibitem{resnet_ref}
K. He, X. Zhang, S. Ren, and J. Sun, ``Deep residual learning for image recognition," \emph{arXiv:1512.03385v1}, Dec. 2015.

\bibitem{beck_fista}
A. Beck and M. Teboulle, ``A fast iterative shrinkage-thresholding algorithm for linear inverse problems," \emph{SIAM J. Imaging Sci.}, vol. 2, no. 1, pp. 183--202, 2009.

\bibitem{sermanet2013overfeat}
P. Sermanet, D. Eigen, X. Zhang, M. Mathieu, R. Fergus, and Y. LeCun, ``Overfeat: Integrated recognition, localization and detection using
convolutional networks." in \emph{Proc. Intl. Conf. on Learning Representations}, 2014.

\bibitem{chen_murphy_deep_cnn}
 L. Chen, G. Papandreou, I. Kokkinos, K. Murphy, and A. L. Yuille, ``Semantic image segmentation with deep convolutional nets and fully
connected CRFs," \emph{arXiv:1412.7062}, 2014. 

\bibitem{hinton2010practical} 
G. Hinton, \emph{Neural Networks: Tricks of the Trade.} $2^{\text{nd}}$ Edition, Springer, Berlin 2012.

\bibitem{rifai2012disentangling}
S. Rifai, Y. Bengio, A. Courville, P. Vincent, and M. Mirza, ``Disentangling factors of variation for facial expression recognition," in \emph{ Proc. European Conf. on Comp. Vis.}, pp. 808--822, 2012.

\bibitem{sutskever2013training}
I. Sutskever, ``Training recurrent neural networks," \emph{Ph.D. dissertation, University of Toronto}, 2013.

\bibitem{ling2015deep}
Z. H. Ling, S. Y. Kang, H. Zen, A. Senior, M. Schuster, X. J. Qian, H. M. Meng, and L. Deng, ``Deep learning for acoustic modeling in parametric
speech generation: A systematic review of existing techniques
and future trends," \emph{IEEE Signal Process. Mag.}, vol. 32, no. 3, pp. 35--52, 2015.

\bibitem{graves2013speech}
A. Graves, A. Mohamed, and G. Hinton, ``Speech recognition with
deep recurrent neural networks," in \emph{Proc. IEEE Intl. Conf. on Acoustics, Speech and Signal Process.}, pp. 6645--6649, 2013.

\bibitem{rifai2012generative}
S. Rifai, Y. Bengio, Y. Dauphin, and P. Vincent, ``A generative process for sampling contractive auto-encoders," \emph{arXiv:1206.6434},
2012.

\bibitem{vincent2010stacked}
P. Vincent, H. Larochelle, I. Lajoie, Y. Bengio, and P. A. Manzagol, ``Stacked denoising auto-encoders: Learning useful representations in a
deep network with a local denoising criterion," \emph{J. Mach. Learn. Res.}, vol. 11, pp. 3371--3408, Dec. 2010.


\bibitem{goodfellow2012large} 
I. Goodfellow, A. Courville, and Y. Bengio, ``Large-scale feature learning with spike-and-slab sparse coding," in \emph{Proc. Intl. Conf. on Machine Learning}, 2012.

\bibitem{lecun_learned_ista}
K. Gregor and Y. LeCun, ``Learning fast approximations of sparse coding," in \emph{Proc. Intl. Conf. on Machine Learning}, 2010.

\bibitem{daubechies_ista}
I. Daubechies, M. Defrise, and C. De Mol, ``An iterative thresholding algorithm for linear inverse problems with a sparsity constraint," \emph{Comm. Pure Appl. Math.}, vol. 57, pp. 1413--1457, 2004.

\bibitem{deep_unfolding_2014}
J.~R.~Hershey, J.~L.~Roux, and F.~Weninger, ``Deep unfolding: Model-based inspiration of novel deep architectures," \emph{arXiv:1409.2575v4}, Nov. 2014.

\bibitem{schniter_lamp}
M. Borgerding, P. Schniter, and S. Rangan, ``AMP-Inspired Deep Networks for Sparse Linear Inverse Problems," \emph{IEEE Trans. Signal Process.}, vol. 65, no. 16, pp. 4293--4308, Aug. 2017.

\bibitem{kamilov_mmse_ista}
U.~S. Kamilov and H.~Mansour, ``Learning optimal nonlinearities for iterative thresholding algorithms,'' \emph{IEEE Signal Process. Letters}, vol.~23, no.~5, pp. 747--751, May 2016.

\bibitem{domke1_cvpr}
J. Domke, ``Parameter learning with truncated message-passing," in \emph{Proc. Comp. Vis. and Pattern Recog.}, pp. 2937--2943, 2011.

\bibitem{domke2_pami}
J. Domke, ``Learning graphical model parameters with approximate marginal inference," \emph{IEEE Trans. Pattern Anal. Mach. Intell.}, vol. 35, no. 10, pp. 24--54, 2013.

\bibitem{sprechmann_sapiro}
P. Sprechmann, A. M. Bronstein, and G. Sapiro, ``Learning efficient sparse and low rank models," \emph{IEEE Trans. Pattern Anal. Mach. Intell.}, vol. 37, no. 5, pp. 1821--1833, Sep. 2015.

\bibitem{wang_l0_encoder}
Z. Wang, Q. Ling, and T. S. Huang, ``Learning deep $\ell_0$ encoders," \emph{arXiv:1509.00153v2}, Nov. 2015.

\bibitem{xin_max_sparsity}
B. Xin, Y. Wang, W. Gao, and D. Wipf, ``Maximal sparsity with deep networks?," \emph{arXiv:1605.01636v2}, May 2016.

\bibitem{jin_et_al}
K. H. Jin, M. T. McCann, E. Froustey, and M. Unser, ``Deep convolutional neural network for inverse problems in imaging," \emph{IEEE Trans. Image Process.}, vol. 26, no. 9, pp. 4509--4522, Sep. 2017.   

\bibitem{ye_et_al}
J. C. Ye and Y. S. Han, ``Deep convolutional framelets: A general deep learning for inverse problems," \emph{arXiv:1707.00372v3}, Aug. 2017.

\bibitem{oktem1}
J. Adler and O. \"Oktem, ``Solving ill-posed inverse problems using iterative deep neural networks," \emph{arXiv:1704.04058v2}, May 2017.

\bibitem{oktem2}
J. Adler and O. \"Oktem, ``Learned primal-dual reconstruction," \emph{arXiv:1707.06474v1}, Jul. 2017.

\bibitem{blu_surelet}
T. Blu and F. Luisier, ``The SURE-LET approach to image denoising," \emph{IEEE Trans. Image Process.}, vol. 16, no. 11, pp. 2778--2786, 2007.


\bibitem{pan2013iterative}
H.~Pan and T.~Blu, ``An iterative linear expansion of thresholds for $\ell_1$-based image restoration,'' \emph{IEEE Trans. Image Process.}, vol.~22, no.~9, pp. 3715--3728, 2013.

\bibitem{martens_hfo}
J.~Martens, ``Deep learning via Hessian-free optimization,'' in \emph{Proc. $27^{\text{th}}$ Intl. Conf. Machine Learning}, pp. 735--742, 2010.

\bibitem{bengio_book}
I. Goodfellow, Y. Bengio, and A. Courville, \emph{Deep learning.}, available at \url{https://www.deeplearningbook.org}.

\bibitem{tibshirani_lasso}
R.Tibshirani, ``Regression shrinkage and selection via the LASSO," \emph{J. Royal Stat. Society, Series B}, vol. 58, no. 1, pp. 267--288, 1996.

\bibitem{parikh_boyd}
N. Parikh and S. Boyd, ``Proximal algorithms," \emph{Foundations and Trends in Opt.}, vol. 1, no. 3, pp. 123--231, 2013.

\bibitem{blu_surelet_deconv}
F. Xue, F. Luisier, and T. Blu, ``Multi-Wiener SURE-LET deconvolution," \emph{IEEE Trans. Image Process.}, vol. 22, no. 5, pp. 1954-1968, 2013.

\bibitem{newsure}
F. Luisier, T. Blu, and M. Unser, ``A new SURE approach to image denoising: Inter-scale orthonormal wavelet thresholding,''
\emph{IEEE Trans. Image Process.} vol. 16, no. 3, pp. 593--606, Mar. 2007.

\bibitem{blu_surelet_tip_2008}
F. Luisier and T. Blu, ``SURE-LET multichannel image denoising: interscale orthonormal wavelet thresholding," \emph{IEEE Trans. Image Process.}, vol. 17, no. 4, pp. 482--492, 2008.

\bibitem{nesterov_momentum1}
Y. E. Nesterov, \emph{Introductory Lectures on Convex Optimization: A Basic Course}, Kluwer Academic Publishers, London, 2004.

\bibitem{pearlmutter1994fast}
B.~A. Pearlmutter, ``Fast exact multiplication by the Hessian,'' \emph{Neural Computation}, vol.~6, no.~1, pp. 147--160, 1994.


\bibitem{fletcher_book}
R. Fletcher, \emph{Practical Methods of Optimization}. $2^{\text{nd}}$ Edition, John Wiley \& Sons, 1987.

%------------------------------------------------------------
%Online RLS references
\bibitem{malioutov_seq_cs_icassp}
D. M. Malioutov, S. Sanghavi, and A. S. Willsky, ``Compressed sensing with sequential observations," in \emph{Proc. IEEE Intl. Conf. on Acoustics, Speech and Signal Process.}, pp. 3357--3360, May 2008.

\bibitem{malioutov_seq_cs}
D. M. Malioutov, S. Sanghavi, and A. S. Willsky, ``Sequential compressed sensing," \emph{arXiv:1003.0219v1}, Mar. 2010. 

\bibitem{asif_romberg}
M. A. Asif and J. Romberg, ``Dynamic updating for $\ell_1$ minimization," \emph{IEEE J. Sel. Topics in Signal Process.}, vol. 4, no.2, pp. 421-434, Apr. 2010.

\bibitem{homotopy1}
P. J. Garrigues and L. E. Ghaoui, ``An homotopy algorithm for the Lasso with online observations," \emph{Adv. in Neural Info. Process. Systems (NIPS)}, pp. 489--496, 2009.

\bibitem{homotopy2}
A. Hofleitner, T. Rabbani, L. E. Ghaoui, and A. Bayen, ``Online homotopy algorithm for a generalization of the LASSO," \emph{IEEE Trans. Automatic Control}, vol. 58, no. 12, pp. 3175-3179, Apr. 2013.

\bibitem{twl}
D. Angelosante, J. A. Bazerque, and G. B. Giannakis, ``Online adaptive estimation of sparse signals: Where RLS meets the $\ell_1$-norm," \emph{IEEE Trans. Signal Process.}, vol. 58, no. 7, pp. 3436--3447, Jul. 2007.

\bibitem{kfcs1}
N. Vaswani, ``Analyzing least squares and Kalman filtered compressed sensing," in \emph{Proc. IEEE Intl. Conf. on Acoustics, Speech and Signal Process.}, pp. 3013--3016, Apr. 2009.

\bibitem{kfcs2}
C. Qiu, W. Lu, and N. Vaswani, ``Real-time dynamic MR image reconstruction using Kalman filtered compressed sensing," in \emph{Proc. IEEE Intl. Conf. on Acoustics, Speech and Signal Process.}, pp. 393--396, Apr. 2009.

\bibitem{distilled_sense1}
J. Haupt, R. Castro, and R. Nowak, ``Distilled sensing: Adaptive sampling for sparse detection and estimation," \emph{IEEE Trans. Info. Theory}, vol. 57, no. 9, pp. 6222--6235, 2011.

\bibitem{distilled_sense2}
J. Haupt, R. Baraniuk, R. Castro, and R. Nowak, ``Sequentially designed compressed sensing," in \emph{Proc. Statistical Signal Process. Workshop}, pp. 401--404, Oct. 2012.

\bibitem{takhar_csim}
D. Takhar, J. N. Laska, M. B. Wakin, M. F. Duarte, D. Baron, S. Sarvotham, K. F. Kelly, and R. G. Baraniuk, ``A new compressive imaging camera architecture using optical-domain compression," in \emph{Proc. SPIE, Computational Imaging IV}, Feb. 2006.


\bibitem{romberg_imaging}
J. Romberg, ``Imaging via compressive sampling," \emph{IEEE Signal Process. Mag.}, vol. 25, no. 2, pp. 14--20, Mar. 2008.

\bibitem{willett}
R. M. Willett, R. F. Marcia, and J. M. Nichols, ``Compressed sensing for practical optical imaging systems: A tutorial," \emph{Optical Engg.}, vol. 50, no. 7, Jul. 2011.

\bibitem{spc}
M. F. Duarte, M. A. Davenport, D. Takhar, J. N. Laska, T. Sun, K. F. Kelly, and R. G. Baraniuk, ``Single-pixel imaging via compressive sampling," \emph{IEEE Signal Process. Mag.}, vol. 25, no. 2, pp. 83--91, Mar. 2008.

\bibitem{csim_color}
P. Nagesh and B. Li, ``Compressive imaging of color images," in \emph{Proc. IEEE Intl. Conf. on Acoustics, Speech and Signal Process.}, pp.  1261--1264, Apr. 2009.

\bibitem{fpa_cs_rice}
H. Chen, M. S. Asif, A. C. Sankaranarayanan, and A. Veeraraghavan, ``FPA-CS: Focal plane array-based compressive imaging in short-wave infrared," in \emph{Proc. Computer Vision and Pattern Recognition}, pp. 2358--2366, 2015.

%------------------------------------------------------------
%Sparse Fienup references
\bibitem{crystallography_chspr}
R. P. Millane, ``Phase retrieval in crystallography and optics," \emph{J. Opt. Soc. Amer. A}, vol. 7, no. 3, pp. 394--411, Mar. 1990.

\bibitem{holography_chspr}
 A. Szoke, ``Holographic microscopy with a complicated reference," \emph{J. Imag. Sci. Technol.}, vol. 41, pp. 332--341, 1997.
 
\bibitem{microscopy_chspr} 
A. J. J. Drenth, A. Huiser, and H. Ferwerda, ``The problem of phase retrieval in light and electron microscopy of strong objects," \emph{Optica Acta}, vol. 22, pp. 615--628, 1975.

\bibitem{fienup_main1}
J. R. Fienup, ``Phase retrieval algorithms: A comparison," \emph{Appl. Opt.}, vol. 21, pp. 2758--2769, 1982.

\bibitem{fienup_main2}
J. R. Fienup, ``Phase retrieval algorithms: A personal tour [invited]," \emph{Appl. Opt.}, vol. 52, pp. 45--56, 2013.

\bibitem{gs_pr}
R. W. Gerchberg and W. O. Saxton, ``A practical algorithm for the determination of phase from image and diffraction plane pictures," \emph{Optik}, vol. 35, pp. 237--246, 1972.

\bibitem{bauschke_pr}
H. H. Bauschke, P. L. Combettes, and D. Luke, ``Phase retrieval, error reduction algorithm, and Fienup variants: A view from convex optimization," \emph{J. Opt. Soc. Amer. A}, vol. 19, pp. 1334--1345, 2002.

\bibitem{quatieri_pr}
T. F. Quatieri and A. V. Oppenheim, ``Iterative techniques for minimum-phase signal reconstruction from phase or magnitude," \emph{IEEE Trans. Acoust., Speech, Signal Process.}, vol. 29, pp. 1187--1193, 1981.

\bibitem{yegna_pr}
B.Yegnanarayana and A. Dhayalan, ``Noniterative techniques for minimum phase signal reconstruction from phase or magnitude," in \emph{Proc. IEEE Intl. Conf. Acoust., Speech, and Signal Process.}, vol. 8, pp. 639--642, Apr. 1983.

\bibitem{css_holography}
C. S. Seelamantula, N. Pavillon, C. Depeursinge, and M. Unser, ``Exact complex-wave reconstruction in digital holography," \emph{J. Opt. Soc. Amer. A}, vol. 28, no. 6, pp. 983--992, Jun. 2011.

\bibitem{param2D_icip}
B. A. Shenoy, S. Mukherjee, and C. S. Seelamantula, ``Phase retrieval for a class of 2-D signals characterized by first-order difference equations," in \emph{Proc. IEEE Intl. Conf. on Image Process.}, pp. 325--329, 2013.

\bibitem{param2D_tip}
B. A. Shenoy and C. S. Seelamantula, ``Exact phase retrieval for a class of 2-D parametric signals," \emph{IEEE Trans. Signal Process.}, vol. 63, no. 1, pp. 90--103, 2015.

\bibitem{pr_shift_invar}
B. A. Shenoy, S. Mulleti, and C. S. Seelamantula, ``Exact phase retrieval in principal shift-invariant spaces," \emph{IEEE Trans. Signal Process.}, vol. 64, no. 2, pp. 406--416, 2016.

\bibitem{moravec_cpr}
M. L. Moravec, J. K. Romberg, and R. G. Baraniuk, ``Compressive phase retrieval," in \emph{Proc. Wavelets XII SPIE Int. Symp. Opt. Sci. Technol.}, Aug. 2007.

\bibitem{yu_vettreli_ssf}
Y. M. Yu and M. Vetterli, ``Sparse spectral factorization: Unicity and reconstruction algorithms," in \emph{Proc. IEEE Intl. Conf. Acoust. Speech, Signal Process.}, pp. 5976--5979, 2011.

\bibitem{gespar}
Y. Shechtman, A. Beck, and Y. C. Eldar, ``GESPAR: Efficient phase retrieval of sparse signals," \emph{IEEE Trans. Signal Process.}, vol. 62, no. 4, pp. 928--938, Feb. 2014. 

\bibitem{netrapalli_altminpr}
P. Netrapalli, P. Jain, and S. Sanghavi, ``Phase retrieval using alternating minimization," \emph{IEEE Trans. Signal Process.}, vol. 63, no. 18, pp. 4814--4826, Sep. 2015.

\bibitem{low_rank_PR_vaswani}
N. Vaswani, S. Nayer, and Y. C. Eldar, ``Low rank phase retrieval," \emph{IEEE Trans. Signal Process.}, vol. 65, no. 15, pp. 4059--4074, Aug. 2017.

\bibitem{dolphin}
A. M. Tillmann, Y. C. Eldar, and J. Mairal, ``DOLPHIn--Dictionary learning for phase retrieval," \emph{IEEE Trans. Signal Process.}, vol. 64, no.
24, pp. 6485--6500, Dec. 2016.

\bibitem{tfocs}
S. Becker, E. J. Cand\`es, and M. Grant, ``Templates for convex cone problems with applications to sparse signal recovery," \emph{Technical Report}, Department of Statistics, Stanford University, 2010.

\bibitem{schniter_gamp}
P. Schniter and S. Rangan, ``Compressive phase retrieval via generalized approximate massage passing," \emph{IEEE Trans. Signal Process.}, vol. 63, no. 4, pp. 1043--1055, Feb. 2015.

\bibitem{bspr_peng}
W. Peng and H. Wang, ``Binary sparse phase retrieval via simulated annealing," \emph{Math. Probl. in Engg.}, Article ID 8257612, May 2016.

\bibitem{palomar_mm}
T. Qiu and D. P. Palomar, ``Undersampled sparse phase retrieval via majorization-minimization," \emph{IEEE Trans. Signal Process.}, vol. 65, no. 22, pp. 5957--5969, Nov. 2017.

\bibitem{fogel_pr_imaging}
F. Fogel, I. Waldspurger, and A. d'Aspremont, ``Phase retrieval for imaging problems," \emph{arXiv:1304.7735v2}, Apr. 2014.

\bibitem{PL1_candes}
E. J. Cand\`es, T. Strohmer, and V. Voroninski, ``PhaseLift: Exact and stable signal recovery from magnitude measurements via convex programming," \emph{Comm. Pure and Appl. Math.}, vol. 66, issue 8, pp. 1241--1274, Aug. 2013.

\bibitem{PL2_candes}
E. J. Cand\`es, Y. C. Eldar, T. Strohmer, and V. Voroninski, ``Phase retrieval via matrix completion," \emph{SIAM J. Imag. Sci.}, vol. 6, issue 1, pp. 199--224, Feb. 2013.  

\bibitem{cpr_pl}
H. Ohlsson, A. Y. Yang, R. Dong, and S. S. Sastry, ``Compressive phase retrieval from squared output measurements via semidefinite programming," \emph{arXiv:1111.6323v3}, Mar. 2012.

\bibitem{qcs_eldar}
Y. Shechtman, Y. C. Eldar, A. Szameit, and M. Segev, ``Sparsity based sub-wavelength imaging with partially incoherent light via quadratic compressed sensing," \emph{Opt. Exp.}, vol. 19, no. 16, pp. 14807--14822, 2011.

\bibitem{power_it}
G. H. Golub and C. H. Van Loan, \emph{Matrix Computations}. $4^{\text{th}}$ Edition, JHU Press, Oct. 1996.

\bibitem{candes_wf_it}
E. J. Cand\`es, X. Li, and M. Soltanolkotabi, ``Phase retrieval via Wirtinger flow: Theory and algorithms," \emph{IEEE Trans. Info. Theory}, vol. 61, no. 4, pp. 1985--2007, Apr. 2015.

\bibitem{candes_twf}
Y. Chen and E. J. Cand\`es, ``Solving random quadratic systems of equations is nearly as easy as solving linear systems," in \emph{Proc. Adv. in Neural Info. Process. Systems (NIPS)}, 2015. 

\bibitem{phasecut}
I. Waldspurger, A. dÕAspremont, and S. Mallat, ``Phase recovery, max-cut and complex semidefinite
programming," \emph{Math. Program.}, vol. 149, no. 1, pp. 47--81, 2015.

\bibitem {luke_pr_diff_image}
D.~R.~Luke, ``Relaxed averaged alternating reflections for diffraction imaging," {\it Inverse Problems}, vol.~21, pp.~37--50, 2005.

\bibitem{oppenheim_dsp_book}
A. V. Oppenheim, R. W. Schaffer, and J. R. Buck, \emph{Discrete-Time Signal Processing}. Prentice Hall, 1998. 

\bibitem{css_oct_2008} 
C.~S.~Seelamantula, M.~L.~Villiger, R.~A.~Leitgeb, and M.~Unser, ``Exact and efficient signal reconstruction in frequency-domain optical coherence tomography," \emph{J. Opt. Soc. Am. (A),} vol.~25, no.~7, pp.~1762--1771, Jul.~2008.

\bibitem{ozcan_oct_2006}
A. Ozcan, M. J. F. Digonnet, and G. S. Kino, ``Minimum-phase-function-based processing in frequency-domain optical-coherence tomography systems," \emph{J. Opt. Soc. Am. A}, vol. 23, pp. 1669--1677, 2006.

\bibitem{css_iisc_journal}
C. S. Seelamantula and T. Lasser, ``Hilbert transform relations in frequency-domain optical-coherence
tomographic imaging," Invited article, \emph{J. Indian Institute of Science, Special issue on Imaging and Microscopy}, vol. 93, no. 1, pp. 139--148, Mar. 2013.

\bibitem{morgan_colormap} 
M. Geissbuehler and T. Lasser, ``How to display data by color schemes compatible with red-green color perception deficiencies,'' \emph{Optics Express}, vol. 21, pp. 9862--9874, 2013.



%-----------QPR references
\bibitem{zymnis_qcs}
A. Zymnis, S. Boyd, and E. J. Cand\`es, ``Compressed sensing with quantized measurements," \emph{IEEE Signal Process. Lett.}, vol. 17, no. 2, pp. 149--152, Feb. 2010. 

\bibitem{laska1}
J. Laska, P. Boufounos, M. Davenport, and R. Baraniuk, ``Democracy in action: Quantization, saturation, and compressive sensing," \emph{Applied and Computational Harmonic Analysis}, vol. 31(3), pp. 429--443, Nov. 2011.

\bibitem{qcs_bit_precision}
E. Ardestanizadeh, M. Cheraghchi, and A. Shokrollahi, ``Bit precision analysis for compressed sensing," in \emph{Proc. IEEE Intl. Symp. on Info. Theory}, pp. 1--5, 2009.

\bibitem{binary_imaging1}
A Bourquard, F. Aguet, and M. Unser, ``Optical imaging using binary sensors," \emph{Opt. Exp.}, vol. 18, no. 5, Mar. 2010.

\bibitem{binary_imaging2}
A Bourquard and M. Unser, ``Binary compressed imaging," \emph{IEEE Trans. Image Process.}, vol. 22, no. 3, pp. 1042--1055, Mar. 2013.

\bibitem{baraniuk1}
P. T. Boufounos and R. G. Baraniuk, ``1-bit compressive sensing," in \emph{Proc. Conf. Info. Science and Systems}, Princeton, NJ, Mar. 2008.

\bibitem{plan1}
Y. Plan and R. Vershynin, ``One-bit compressed sensing by linear programming," \emph{arXiv:1109.4299v5}, Mar. 2012.

\bibitem{msp}
P. T. Boufounos, ``Greedy sparse signal reconstruction from sign measurements," in \emph{Proc. Asilomar Conf.  Signals, Systems, and Computation}, Asilomar, CA, Nov. 2009.

\bibitem{var_gamma_ref}
D.B. Madan and E. Seneta, ``The variance gamma (V.G.) model for share market returns," \emph{J. Business}, vol. 63, no. 4, pp. 511--524, Oct. 1990.

\bibitem{jayant_noll}
N. S. Jayant and P. Noll, \textit{Digital Coding of Waveforms: Principles and Applications to Speech and Video}. Prentice-Hall, USA, 1984.

\bibitem{bstj_paper}
B. Smith, ``Instantaneous companding of quantized signals," \emph{Bell System Tech. J.}, vol. 36, pp. 653--709, May 1957.


\bibitem{svt_candes}
J.-F. Cai, E. J. Cand\`es, and Z. Shen, ``A singular value thresholding algorithm for matrix completion," \emph{SIAM J. Optimization}, vol. 20, no. 4, pp. 1956--1982, Mar. 2010.


\bibitem{geng_yang}
J. Geng, X. Yang, X. Wang, and L. Wang, ``An accelerated iterative hard-thresholding method for matrix completion," \emph{Intl. J. Signal Process., Image Process., and Pattern Recog.}, vol. 8, no. 7, pp. 141--150, 2015.

\bibitem{balan1_qpr}
R. Balan, ``Reconstruction of signals from magnitudes of redundant representations: The complex case," \emph{Found. Comp. Math.}, pp. 1--45, 2013.
 
\bibitem{balan2_qpr}
R. Balan, ``The Fisher information matrix and the CRLB in a non-AWGN model for the phase retrieval problem," in \emph{Proc. Intl. Conf. Sampl. Theory and Applications}, pp. 178--182, 2015. 

\bibitem{pr_crb_fpp_qpr}
C. Qian, N. D. Sidiropoulos, K. Huang, L. Huang, and H. C. So, ``Phase retrieval using feasible point pursuit: Algorithms and Cram\'er-Rao bound," \emph{IEEE Trans. Signal Process.}, vol. 64, no. 20, pp. 5282--5296, Oct. 2016.

\bibitem{bandeira_qpr}
 A. S. Bandeira, J. Cahill, D. G. Mixon, and A. A. Nelson, ``Saving phase: Injectivity and stability for phase retrieval," \emph{Appl. and Comp. Harmonic Anal.}, vol. 37, no. 1, pp. 106--125, 2014.

\bibitem{cederquist_qpr}
J. N. Cederquist and C. C. Wackerman, ``Phase-retrieval error: A lower bound," \emph{J. Opt. Soc. Amer. A}, vol. 4, no. 9, pp. 1788--1792, 1987.


\end{thebibliography}

